Learn the Time to Learn: Replay Scheduling in Continual Learning

Replay methods are known to be successful at mitigating catastrophic forgetting in continual learning scenarios despite having limited access to historical data. However, storing historical data is cheap in many real-world settings, yet replaying all historical data is often prohibited due to processing time constraints. In such settings, we propose that continual learning systems should learn the time to learn and schedule which tasks to replay at different time steps. We first demonstrate the benefits of our proposal by using Monte Carlo tree search to find a proper replay schedule, and show that the found replay schedules can outperform fixed scheduling policies when combined with various replay methods in different continual learning settings. Additionally, we propose a framework for learning replay scheduling policies with reinforcement learning. We show that the learned policies can generalize better in new continual learning scenarios compared to equally replaying all seen tasks, without added computational cost. Our study reveals the importance of learning the time to learn in continual learning, which brings current research closer to real-world needs.

==> figures/acc_over_memory_size_100iters/CIFAR100_acc_over_memory.tex <==

\nextgroupplot[title=Split CIFAR-100,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={95,285,475,950,1900},
y grid style={white!69.0196078431373!black},
ymajorgrids,
%ylabel={ACC},
ymin=0.495, ymax=0.810957793848251,
ytick style={color=black},
ytick={0.5, 0.55, 0.6,0.65,0.7,0.75,0.8,0.85},
yticklabels={50, 55, 60, 65, 70, 75, 80, 85}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.562037039718105)
--(axis cs:1,0.576362960281895)
--(axis cs:2,0.689751105919972)
--(axis cs:3,0.721032799845321)
--(axis cs:4,0.758455325125059)
--(axis cs:5,0.792425179734339)
--(axis cs:5,0.784774820265661)
--(axis cs:5,0.784774820265661)
--(axis cs:4,0.749304674874941)
--(axis cs:3,0.696207200154679)
--(axis cs:2,0.665968894080028)
--(axis cs:1,0.562037039718105)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.54420843806795)
--(axis cs:1,0.55951156193205)
--(axis cs:2,0.660018780412226)
--(axis cs:3,0.701282341220295)
--(axis cs:4,0.74849294674193)
--(axis cs:5,0.780335209714517)
--(axis cs:5,0.772824790285483)
--(axis cs:5,0.772824790285483)
--(axis cs:4,0.73630705325807)
--(axis cs:3,0.686757658779705)
--(axis cs:2,0.640341219587774)
--(axis cs:1,0.54420843806795)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.499704018706963)
--(axis cs:1,0.577535981293037)
--(axis cs:2,0.631322030526373)
--(axis cs:3,0.68081333911034)
--(axis cs:4,0.714779020310597)
--(axis cs:5,0.698210881385584)
--(axis cs:5,0.575789118614416)
--(axis cs:5,0.575789118614416)
--(axis cs:4,0.604540979689403)
--(axis cs:3,0.61926666088966)
--(axis cs:2,0.573797969473627)
--(axis cs:1,0.499704018706963)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.594093382358551)
--(axis cs:1,0.615146577358246)
--(axis cs:2,0.694118440151215)
--(axis cs:3,0.734759986400604)
--(axis cs:4,0.772708475589752)
--(axis cs:5,0.798255443572998)
--(axis cs:5,0.786504507064819)
--(axis cs:5,0.786504507064819)
--(axis cs:4,0.760211646556854)
--(axis cs:3,0.723879992961884)
--(axis cs:2,0.682881414890289)
--(axis cs:1,0.594093382358551)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.581120014190674
2 0.675799965858459
3 0.716120004653931
4 0.754159986972809
5 0.786180078983307
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.5692
2 0.67786
3 0.70862
4 0.75388
5 0.7886
};

\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.53862
2 0.60256
3 0.65004
4 0.65966
5 0.637
};

\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.604619979858398
2 0.688499927520752
3 0.729319989681244
4 0.766460061073303
5 0.792379975318909
};




==> figures/acc_over_memory_size_100iters/FashionMNIST_acc_over_memory.tex <==

\nextgroupplot[title=Split FashionMNIST,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.89, 0.91, 0.93, 0.95, 0.97, 0.99},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
%xlabel={Memory size \(\displaystyle M\)},
xmin=0.7, xmax=7.3,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=90},
xticklabels={8,24,80,120,200,400,800},
y grid style={white!69.0196078431373!black},
ymajorgrids,
yminorgrids,
%ylabel={ACC},
ymin=0.899,%0.891766529814355,
ymax=0.996494715797058,
ytick style={color=black},
ytick={0.88,0.9,0.92,0.94,0.96,0.98,1},
yticklabels={88, 90, 92, 94, 96, 98, 100}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.926061224352897)
--(axis cs:1,0.974738775647103)
--(axis cs:2,0.979121260392956)
--(axis cs:3,0.98438381267246)
--(axis cs:4,0.987243668181702)
--(axis cs:5,1.00007329259331)
--(axis cs:6,0.995954220056289)
--(axis cs:7,1.00924829851241)
--(axis cs:7,0.930671701487593)
--(axis cs:7,0.930671701487593)
--(axis cs:6,0.964125779943711)
--(axis cs:5,0.93352670740669)
--(axis cs:4,0.978516331818298)
--(axis cs:3,0.95269618732754)
--(axis cs:2,0.964838739607044)
--(axis cs:1,0.926061224352897)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.965724160568608)
--(axis cs:1,0.979275839431391)
--(axis cs:2,0.983843648420532)
--(axis cs:3,0.987767732323772)
--(axis cs:4,0.988072744085454)
--(axis cs:5,0.988506841180757)
--(axis cs:6,0.989178836422143)
--(axis cs:7,0.990307375485654)
--(axis cs:7,0.989052624514346)
--(axis cs:7,0.989052624514346)
--(axis cs:6,0.987461163577857)
--(axis cs:5,0.983413158819243)
--(axis cs:4,0.982567255914546)
--(axis cs:3,0.970792267676228)
--(axis cs:2,0.972876351579468)
--(axis cs:1,0.965724160568608)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.955000050761585)
--(axis cs:1,0.970759949238415)
--(axis cs:2,0.98603178628668)
--(axis cs:3,0.981832320290786)
--(axis cs:4,0.983967730086771)
--(axis cs:5,0.978253058795492)
--(axis cs:6,0.991734343706935)
--(axis cs:7,0.969833098095523)
--(axis cs:7,0.896526901904478)
--(axis cs:7,0.896526901904478)
--(axis cs:6,0.916425656293065)
--(axis cs:5,0.938266941204508)
--(axis cs:4,0.921192269913229)
--(axis cs:3,0.942567679709214)
--(axis cs:2,0.92920821371332)
--(axis cs:1,0.955000050761585)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.982129275798798)
--(axis cs:1,0.984390676021576)
--(axis cs:2,0.987218379974365)
--(axis cs:3,0.988464534282684)
--(axis cs:4,0.989360094070435)
--(axis cs:5,0.989464402198792)
--(axis cs:6,0.989146828651428)
--(axis cs:7,0.990860760211945)
--(axis cs:7,0.988419115543365)
--(axis cs:7,0.988419115543365)
--(axis cs:6,0.98689329624176)
--(axis cs:5,0.987175583839417)
--(axis cs:4,0.985639929771423)
--(axis cs:3,0.983615458011627)
--(axis cs:2,0.982341647148132)
--(axis cs:1,0.982129275798798)
--cycle;
\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.9504
2 0.97198
3 0.96854
4 0.98288
5 0.9668
6 0.98004
7 0.96996
};
%\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.9725
2 0.97836
3 0.97928
4 0.98532
5 0.98596
6 0.98832
7 0.98968
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.96288
2 0.95762
3 0.9622
4 0.95258
5 0.95826
6 0.95408
7 0.93318
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.983259975910187
2 0.984780013561249
3 0.986039996147156
4 0.987500011920929
5 0.988319993019104
6 0.988020062446594
7 0.989639937877655
};
%\addlegendentry{Ours}



==> figures/acc_over_memory_size_100iters/MNIST_acc_over_memory.tex <==
\nextgroupplot[title=Split MNIST,
height=\figheight,
legend cell align={left},
%legend style={
%  nodes={scale=1.0},%=0.95},%{scale=0.9},
%  fill opacity=0.8,
%  draw opacity=1,
%  text opacity=1,
%  at={(3.90,-0.15)}, %{(3.70,-0.30)},   %{(3.72,0.13)},
%  anchor=south west,
%  draw=white!80!black
%},
legend columns=-1,
legend style={
  nodes={scale=0.85},%=0.95},%{scale=0.9},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,1.28)}, %{(3.70,-0.30)},   %{(3.72,0.13)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
%xlabel={Memory size \(\displaystyle M\)},
xmin=0.7, xmax=7.3,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=90},
xticklabels={8,24,80,120,200,400,800},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ylabel={ACC (\%)},
ymin=0.939, ymax=0.997729043511215,
ytick style={color=black},
ytick={0.92,0.93,0.94,0.95,0.96,0.97,0.98,0.99,1},
yticklabels={92,93,94,95,96,97,98,99,100}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.9358148518719)
--(axis cs:1,0.9741387481281)
--(axis cs:2,0.989098536355273)
--(axis cs:3,0.995966564108866)
--(axis cs:4,1.00110431438662)
--(axis cs:5,0.995835486970184)
--(axis cs:6,1.00211387317156)
--(axis cs:7,1.0002227112054)
--(axis cs:7,0.971772728794604)
--(axis cs:7,0.971772728794604)
--(axis cs:6,0.957473726828435)
--(axis cs:5,0.963949953029816)
--(axis cs:4,0.955316885613383)
--(axis cs:3,0.955402955891134)
--(axis cs:2,0.955082823644727)
--(axis cs:1,0.9358148518719)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.946015386753438)
--(axis cs:1,0.970621573246562)
--(axis cs:2,0.984533286206628)
--(axis cs:3,0.988692537329328)
--(axis cs:4,0.990023216819651)
--(axis cs:5,0.990669279851693)
--(axis cs:6,0.992800317892538)
--(axis cs:7,0.994021984494329)
--(axis cs:7,0.992872175505671)
--(axis cs:7,0.992872175505671)
--(axis cs:6,0.990845362107462)
--(axis cs:5,0.986030240148307)
--(axis cs:4,0.986402863180349)
--(axis cs:3,0.980789062670673)
--(axis cs:2,0.972900553793372)
--(axis cs:1,0.946015386753438)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.953295697386423)
--(axis cs:1,0.969893182613577)
--(axis cs:2,0.989900327489411)
--(axis cs:3,0.987615676138068)
--(axis cs:4,0.987468694435405)
--(axis cs:5,0.987904186526891)
--(axis cs:6,0.990390603540462)
--(axis cs:7,0.991611458769248)
--(axis cs:7,0.983504221230752)
--(axis cs:7,0.983504221230752)
--(axis cs:6,0.978347876459538)
--(axis cs:5,0.975166293473109)
--(axis cs:4,0.979932985564595)
--(axis cs:3,0.979642883861932)
--(axis cs:2,0.966454952510589)
--(axis cs:1,0.953295697386423)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.976848125457764)
--(axis cs:1,0.986456036567688)
--(axis cs:2,0.988981068134308)
--(axis cs:3,0.992213249206543)
--(axis cs:4,0.991635799407959)
--(axis cs:5,0.991742670536041)
--(axis cs:6,0.992980241775513)
--(axis cs:7,0.994612276554108)
--(axis cs:7,0.993073880672455)
--(axis cs:7,0.993073880672455)
--(axis cs:6,0.992027640342712)
--(axis cs:5,0.990043103694916)
--(axis cs:4,0.989341855049133)
--(axis cs:3,0.989036798477173)
--(axis cs:2,0.982677280902863)
--(axis cs:1,0.976848125457764)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.9549768
2 0.97209068
3 0.97568476
4 0.9782106
5 0.97989272
6 0.9797938
7 0.98599772
};
\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.95831848
2 0.97871692
3 0.9847408
4 0.98821304
5 0.98834976
6 0.99182284
7 0.99344708
};\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.96159444
2 0.97817764
3 0.98362928
4 0.98370084
5 0.98153524
6 0.98436924
7 0.98755784
};
\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.981652081012726
2 0.985829174518585
3 0.990625023841858
4 0.990488827228546
5 0.990892887115479
6 0.992503941059113
7 0.993843078613281
};\addlegendentry{Ours}




==> figures/acc_over_memory_size_100iters/PermutedMNIST_acc_over_memory.tex <==
\nextgroupplot[title=Permuted MNIST,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={90,270,450,900,2250},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ylabel={ACC (\%)},
ymin=0.695,%0.637838739156723, 
ymax=0.93909129061632,
ytick style={color=black},
ytick={0.60,0.65,0.7,0.75,0.8,0.85,0.9,0.95},
yticklabels={60,65,70,75,80,85,90,95}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.715730226321196)
--(axis cs:1,0.736885773678804)
--(axis cs:2,0.827973539580458)
--(axis cs:3,0.861050780378148)
--(axis cs:4,0.890440219509845)
--(axis cs:5,0.913933024403524)
--(axis cs:5,0.904794975596476)
--(axis cs:5,0.904794975596476)
--(axis cs:4,0.869939780490155)
--(axis cs:3,0.833253219621852)
--(axis cs:2,0.812214460419542)
--(axis cs:1,0.715730226321196)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.703322259916344)
--(axis cs:1,0.726421740083656)
--(axis cs:2,0.813376771868685)
--(axis cs:3,0.855015954553463)
--(axis cs:4,0.884852627163868)
--(axis cs:5,0.912982539743805)
--(axis cs:5,0.908409460256195)
--(axis cs:5,0.908409460256195)
--(axis cs:4,0.875559372836131)
--(axis cs:3,0.832572045446536)
--(axis cs:2,0.800187228131315)
--(axis cs:1,0.703322259916344)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.738538401173349)
--(axis cs:1,0.771401598826651)
--(axis cs:2,0.798919804972782)
--(axis cs:3,0.839665791039941)
--(axis cs:4,0.835268339924516)
--(axis cs:5,0.850651036649128)
--(axis cs:5,0.774932963350872)
--(axis cs:5,0.774932963350872)
--(axis cs:4,0.770147660075484)
--(axis cs:3,0.793590208960059)
--(axis cs:2,0.767396195027218)
--(axis cs:1,0.738538401173349)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.709841430187225)
--(axis cs:1,0.723326504230499)
--(axis cs:2,0.824357867240906)
--(axis cs:3,0.859517455101013)
--(axis cs:4,0.893725514411926)
--(axis cs:5,0.927864193916321)
--(axis cs:5,0.921083688735962)
--(axis cs:5,0.921083688735962)
--(axis cs:4,0.88515043258667)
--(axis cs:3,0.851162552833557)
--(axis cs:2,0.817286252975464)
--(axis cs:1,0.709841430187225)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.726308
2 0.820094
3 0.847152
4 0.88019
5 0.909364
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.714872
2 0.806782
3 0.843794
4 0.880206
5 0.910696
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.75497
2 0.783158
3 0.816628
4 0.802708
5 0.812792
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.716583967208862
2 0.820822060108185
3 0.855340003967285
4 0.889437973499298
5 0.924473941326141
};
%\addlegendentry{Ours}


==> figures/acc_over_memory_size_100iters/acc_over_memory_size_groupplot.tex <==



\pgfplotsset{every axis title/.append style={at={(0.5,0.80)}}} %{at={(0.5,0.84)}}}
\pgfplotsset{every tick label/.append style={font=\tiny}}
\pgfplotsset{every major tick/.append style={major tick length=2pt}}
\pgfplotsset{every minor tick/.append style={minor tick length=1pt}}
\pgfplotsset{every axis x label/.append style={at={(0.5,-0.27)}}}
\pgfplotsset{every axis y label/.append style={at={(-0.20,0.5)}}}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{groupplot}[group style={group size= 3 by 2, horizontal sep=0.9cm, vertical sep=0.9cm}]

\input{figures/acc_over_memory_size_100iters/MNIST_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/FashionMNIST_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/notMNIST_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/PermutedMNIST_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/CIFAR100_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/miniImagenet_acc_over_memory}

\end{groupplot}

\end{tikzpicture}

==> figures/acc_over_memory_size_100iters/miniImagenet_acc_over_memory.tex <==

\nextgroupplot[title=Split miniImagenet,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.525, 0.575, 0.625, 0.675},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={95,285,475,950,1900},
y grid style={white!69.0196078431373!black},
ymajorgrids, yminorgrids,
%ylabel={ACC},
ymin=0.485468408535527, ymax=0.656408178377217,
ytick style={color=black},
ytick={0.5,0.55,0.6,0.65,0.70},
yticklabels={50,55,60,65,70}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.511239936034333)
--(axis cs:1,0.530000063965667)
--(axis cs:2,0.589402344070757)
--(axis cs:3,0.607880865354614)
--(axis cs:4,0.627174196127067)
--(axis cs:5,0.636374896060481)
--(axis cs:5,0.622665103939519)
--(axis cs:5,0.622665103939519)
--(axis cs:4,0.610225803872933)
--(axis cs:3,0.582919134645386)
--(axis cs:2,0.567557655929243)
--(axis cs:1,0.511239936034333)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.493238398073785)
--(axis cs:1,0.533441601926215)
--(axis cs:2,0.57011855059778)
--(axis cs:3,0.605819593487538)
--(axis cs:4,0.614540951326373)
--(axis cs:5,0.630535426185857)
--(axis cs:5,0.616984573814143)
--(axis cs:5,0.616984573814143)
--(axis cs:4,0.595619048673627)
--(axis cs:3,0.586140406512462)
--(axis cs:2,0.55356144940222)
--(axis cs:1,0.493238398073785)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.492947858361007)
--(axis cs:1,0.520172141638993)
--(axis cs:2,0.555463345135852)
--(axis cs:3,0.547130468985637)
--(axis cs:4,0.556312161267811)
--(axis cs:5,0.595653887589556)
--(axis cs:5,0.532706112410444)
--(axis cs:5,0.532706112410444)
--(axis cs:4,0.463447838732189)
--(axis cs:3,0.455229531014363)
--(axis cs:2,0.511216654864149)
--(axis cs:1,0.492947858361007)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.533491373062134)
--(axis cs:1,0.538228631019592)
--(axis cs:2,0.57997077703476)
--(axis cs:3,0.604763567447662)
--(axis cs:4,0.625060558319092)
--(axis cs:5,0.648638188838959)
--(axis cs:5,0.627881824970245)
--(axis cs:5,0.627881824970245)
--(axis cs:4,0.611339330673218)
--(axis cs:3,0.595156371593475)
--(axis cs:2,0.578189194202423)
--(axis cs:1,0.533491373062134)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.52062
2 0.57848
3 0.5954
4 0.6187
5 0.62952
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.51334
2 0.56184
3 0.59598
4 0.60508
5 0.62376
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.50656
2 0.53334
3 0.50118
4 0.50988
5 0.56418
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.535860002040863
2 0.579079985618591
3 0.599959969520569
4 0.618199944496155
5 0.638260006904602
};
%\addlegendentry{RS-MCTS}





==> figures/acc_over_memory_size_100iters/notMNIST_acc_over_memory.tex <==
\nextgroupplot[title=Split notMNIST,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.91, 0.93, 0.95, 0.97},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
%xlabel={Memory size \(\displaystyle M\)},
xmin=0.7, xmax=7.3,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=90},
xticklabels={8,24,80,120,200,400,800},
y grid style={white!69.0196078431373!black},
ymajorgrids,
yminorgrids,
%ylabel={ACC},
ymin=0.899, ymax=0.968037298370892,
ytick style={color=black},
ytick={0.9,0.92,0.94,0.96,0.98},
yticklabels={90, 92, 94, 96, 98}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.896013207305508)
--(axis cs:1,0.931135192694492)
--(axis cs:2,0.938159623242489)
--(axis cs:3,0.950881648994029)
--(axis cs:4,0.959366722972026)
--(axis cs:5,0.953366381554805)
--(axis cs:6,0.957957912748783)
--(axis cs:7,0.956996714641506)
--(axis cs:7,0.942492645358494)
--(axis cs:7,0.942492645358494)
--(axis cs:6,0.935719447251217)
--(axis cs:5,0.925448018445195)
--(axis cs:4,0.938790317027974)
--(axis cs:3,0.931924351005971)
--(axis cs:2,0.908068296757511)
--(axis cs:1,0.896013207305508)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.905642837956127)
--(axis cs:1,0.936302282043873)
--(axis cs:2,0.945930444061739)
--(axis cs:3,0.952986088925952)
--(axis cs:4,0.959824157530047)
--(axis cs:5,0.952829054017519)
--(axis cs:6,0.959656752670672)
--(axis cs:7,0.962564882794123)
--(axis cs:7,0.947773837205876)
--(axis cs:7,0.947773837205876)
--(axis cs:6,0.948538687329328)
--(axis cs:5,0.942894385982481)
--(axis cs:4,0.946525122469953)
--(axis cs:3,0.939538551074048)
--(axis cs:2,0.917796675938261)
--(axis cs:1,0.905642837956127)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.92575112968193)
--(axis cs:1,0.94785415031807)
--(axis cs:2,0.955205714329457)
--(axis cs:3,0.958007719572493)
--(axis cs:4,0.952085855254064)
--(axis cs:5,0.955086757682649)
--(axis cs:6,0.947191690371997)
--(axis cs:7,0.964993528242304)
--(axis cs:7,0.936188951757696)
--(axis cs:7,0.936188951757696)
--(axis cs:6,0.909628229628003)
--(axis cs:5,0.922580682317351)
--(axis cs:4,0.916396464745937)
--(axis cs:3,0.906849720427507)
--(axis cs:2,0.904118125670543)
--(axis cs:1,0.92575112968193)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.939071178436279)
--(axis cs:1,0.951526403427124)
--(axis cs:2,0.958871364593506)
--(axis cs:3,0.954144775867462)
--(axis cs:4,0.952358484268188)
--(axis cs:5,0.95714259147644)
--(axis cs:6,0.956836819648743)
--(axis cs:7,0.9615877866745)
--(axis cs:7,0.9475919008255)
--(axis cs:7,0.9475919008255)
--(axis cs:6,0.94806444644928)
--(axis cs:5,0.94659161567688)
--(axis cs:4,0.93076229095459)
--(axis cs:3,0.942625343799591)
--(axis cs:2,0.945715665817261)
--(axis cs:1,0.939071178436279)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.9135742
2 0.92311396
3 0.941403
4 0.94907852
5 0.9394072
6 0.94683868
7 0.94974468
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.92097256
2 0.93186356
3 0.94626232
4 0.95317464
5 0.94786172
6 0.95409772
7 0.95516936
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.93680264
2 0.92966192
3 0.93242872
4 0.93424116
5 0.93883372
6 0.92840996
7 0.95059124
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.945298790931702
2 0.952293515205383
3 0.948385059833527
4 0.941560387611389
5 0.95186710357666
6 0.952450633049011
7 0.95458984375
};
%\addlegendentry{RS-MCTS}



==> figures/acc_over_memory_size_100iters_new/CIFAR100_acc_over_memory.tex <==

\nextgroupplot[title=Split CIFAR-100,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=90},
xticklabels={95,285,475,950,1900},
y grid style={white!69.0196078431373!black},
ymajorgrids,
%ylabel={ACC},
ymin=0.495, ymax=0.810957793848251,
ytick style={color=black},
ytick={0.5, 0.55, 0.6,0.65,0.7,0.75,0.8,0.85},
yticklabels={50, 55, 60, 65, 70, 75, 80, 85}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.562037039718105)
--(axis cs:1,0.576362960281895)
--(axis cs:2,0.689751105919972)
--(axis cs:3,0.721032799845321)
--(axis cs:4,0.758455325125059)
--(axis cs:5,0.792425179734339)
--(axis cs:5,0.784774820265661)
--(axis cs:5,0.784774820265661)
--(axis cs:4,0.749304674874941)
--(axis cs:3,0.696207200154679)
--(axis cs:2,0.665968894080028)
--(axis cs:1,0.562037039718105)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.54420843806795)
--(axis cs:1,0.55951156193205)
--(axis cs:2,0.660018780412226)
--(axis cs:3,0.701282341220295)
--(axis cs:4,0.74849294674193)
--(axis cs:5,0.780335209714517)
--(axis cs:5,0.772824790285483)
--(axis cs:5,0.772824790285483)
--(axis cs:4,0.73630705325807)
--(axis cs:3,0.686757658779705)
--(axis cs:2,0.640341219587774)
--(axis cs:1,0.54420843806795)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.499704018706963)
--(axis cs:1,0.577535981293037)
--(axis cs:2,0.631322030526373)
--(axis cs:3,0.68081333911034)
--(axis cs:4,0.714779020310597)
--(axis cs:5,0.698210881385584)
--(axis cs:5,0.575789118614416)
--(axis cs:5,0.575789118614416)
--(axis cs:4,0.604540979689403)
--(axis cs:3,0.61926666088966)
--(axis cs:2,0.573797969473627)
--(axis cs:1,0.499704018706963)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.594093382358551)
--(axis cs:1,0.615146577358246)
--(axis cs:2,0.694118440151215)
--(axis cs:3,0.734759986400604)
--(axis cs:4,0.772708475589752)
--(axis cs:5,0.798255443572998)
--(axis cs:5,0.786504507064819)
--(axis cs:5,0.786504507064819)
--(axis cs:4,0.760211646556854)
--(axis cs:3,0.723879992961884)
--(axis cs:2,0.682881414890289)
--(axis cs:1,0.594093382358551)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.581120014190674
2 0.675799965858459
3 0.716120004653931
4 0.754159986972809
5 0.786180078983307
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.5692
2 0.67786
3 0.70862
4 0.75388
5 0.7886
};

\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.53862
2 0.60256
3 0.65004
4 0.65966
5 0.637
};

\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.604619979858398
2 0.688499927520752
3 0.729319989681244
4 0.766460061073303
5 0.792379975318909
};




==> figures/acc_over_memory_size_100iters_new/FashionMNIST_acc_over_memory.tex <==

\nextgroupplot[title=Split FashionMNIST,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.89, 0.91, 0.93, 0.95, 0.97, 0.99},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
%xlabel={Memory size \(\displaystyle M\)},
xmin=0.7, xmax=7.3,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=90},
xticklabels={8,24,80,120,200,400,800},
y grid style={white!69.0196078431373!black},
ymajorgrids,
yminorgrids,
%ylabel={ACC},
ymin=0.899,%0.891766529814355,
ymax=0.996494715797058,
ytick style={color=black},
ytick={0.88,0.9,0.92,0.94,0.96,0.98,1},
yticklabels={88, 90, 92, 94, 96, 98, 100}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.926061224352897)
--(axis cs:1,0.974738775647103)
--(axis cs:2,0.979121260392956)
--(axis cs:3,0.98438381267246)
--(axis cs:4,0.987243668181702)
--(axis cs:5,1.00007329259331)
--(axis cs:6,0.995954220056289)
--(axis cs:7,1.00924829851241)
--(axis cs:7,0.930671701487593)
--(axis cs:7,0.930671701487593)
--(axis cs:6,0.964125779943711)
--(axis cs:5,0.93352670740669)
--(axis cs:4,0.978516331818298)
--(axis cs:3,0.95269618732754)
--(axis cs:2,0.964838739607044)
--(axis cs:1,0.926061224352897)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.965724160568608)
--(axis cs:1,0.979275839431391)
--(axis cs:2,0.983843648420532)
--(axis cs:3,0.987767732323772)
--(axis cs:4,0.988072744085454)
--(axis cs:5,0.988506841180757)
--(axis cs:6,0.989178836422143)
--(axis cs:7,0.990307375485654)
--(axis cs:7,0.989052624514346)
--(axis cs:7,0.989052624514346)
--(axis cs:6,0.987461163577857)
--(axis cs:5,0.983413158819243)
--(axis cs:4,0.982567255914546)
--(axis cs:3,0.970792267676228)
--(axis cs:2,0.972876351579468)
--(axis cs:1,0.965724160568608)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.955000050761585)
--(axis cs:1,0.970759949238415)
--(axis cs:2,0.98603178628668)
--(axis cs:3,0.981832320290786)
--(axis cs:4,0.983967730086771)
--(axis cs:5,0.978253058795492)
--(axis cs:6,0.991734343706935)
--(axis cs:7,0.969833098095523)
--(axis cs:7,0.896526901904478)
--(axis cs:7,0.896526901904478)
--(axis cs:6,0.916425656293065)
--(axis cs:5,0.938266941204508)
--(axis cs:4,0.921192269913229)
--(axis cs:3,0.942567679709214)
--(axis cs:2,0.92920821371332)
--(axis cs:1,0.955000050761585)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.982129275798798)
--(axis cs:1,0.984390676021576)
--(axis cs:2,0.987218379974365)
--(axis cs:3,0.988464534282684)
--(axis cs:4,0.989360094070435)
--(axis cs:5,0.989464402198792)
--(axis cs:6,0.989146828651428)
--(axis cs:7,0.990860760211945)
--(axis cs:7,0.988419115543365)
--(axis cs:7,0.988419115543365)
--(axis cs:6,0.98689329624176)
--(axis cs:5,0.987175583839417)
--(axis cs:4,0.985639929771423)
--(axis cs:3,0.983615458011627)
--(axis cs:2,0.982341647148132)
--(axis cs:1,0.982129275798798)
--cycle;
\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.9504
2 0.97198
3 0.96854
4 0.98288
5 0.9668
6 0.98004
7 0.96996
};
%\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.9725
2 0.97836
3 0.97928
4 0.98532
5 0.98596
6 0.98832
7 0.98968
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.96288
2 0.95762
3 0.9622
4 0.95258
5 0.95826
6 0.95408
7 0.93318
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.983259975910187
2 0.984780013561249
3 0.986039996147156
4 0.987500011920929
5 0.988319993019104
6 0.988020062446594
7 0.989639937877655
};
%\addlegendentry{Ours}



==> figures/acc_over_memory_size_100iters_new/MNIST_acc_over_memory.tex <==
\nextgroupplot[title=Split MNIST,
height=\figheight,
legend cell align={left},
%legend style={
%  nodes={scale=1.0},%=0.95},%{scale=0.9},
%  fill opacity=0.8,
%  draw opacity=1,
%  text opacity=1,
%  at={(3.90,-0.15)}, %{(3.70,-0.30)},   %{(3.72,0.13)},
%  anchor=south west,
%  draw=white!80!black
%},
legend columns=-1,
legend style={
  nodes={scale=0.85},%=0.95},%{scale=0.9},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,1.28)}, %{(3.70,-0.30)},   %{(3.72,0.13)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
%xlabel={Memory size \(\displaystyle M\)},
xmin=0.7, xmax=7.3,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=90},
xticklabels={8,24,80,120,200,400,800},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ylabel={ACC (\%)},
ymin=0.939, ymax=0.997729043511215,
ytick style={color=black},
ytick={0.92,0.93,0.94,0.95,0.96,0.97,0.98,0.99,1},
yticklabels={92,93,94,95,96,97,98,99,100}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.9358148518719)
--(axis cs:1,0.9741387481281)
--(axis cs:2,0.989098536355273)
--(axis cs:3,0.995966564108866)
--(axis cs:4,1.00110431438662)
--(axis cs:5,0.995835486970184)
--(axis cs:6,1.00211387317156)
--(axis cs:7,1.0002227112054)
--(axis cs:7,0.971772728794604)
--(axis cs:7,0.971772728794604)
--(axis cs:6,0.957473726828435)
--(axis cs:5,0.963949953029816)
--(axis cs:4,0.955316885613383)
--(axis cs:3,0.955402955891134)
--(axis cs:2,0.955082823644727)
--(axis cs:1,0.9358148518719)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.946015386753438)
--(axis cs:1,0.970621573246562)
--(axis cs:2,0.984533286206628)
--(axis cs:3,0.988692537329328)
--(axis cs:4,0.990023216819651)
--(axis cs:5,0.990669279851693)
--(axis cs:6,0.992800317892538)
--(axis cs:7,0.994021984494329)
--(axis cs:7,0.992872175505671)
--(axis cs:7,0.992872175505671)
--(axis cs:6,0.990845362107462)
--(axis cs:5,0.986030240148307)
--(axis cs:4,0.986402863180349)
--(axis cs:3,0.980789062670673)
--(axis cs:2,0.972900553793372)
--(axis cs:1,0.946015386753438)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.953295697386423)
--(axis cs:1,0.969893182613577)
--(axis cs:2,0.989900327489411)
--(axis cs:3,0.987615676138068)
--(axis cs:4,0.987468694435405)
--(axis cs:5,0.987904186526891)
--(axis cs:6,0.990390603540462)
--(axis cs:7,0.991611458769248)
--(axis cs:7,0.983504221230752)
--(axis cs:7,0.983504221230752)
--(axis cs:6,0.978347876459538)
--(axis cs:5,0.975166293473109)
--(axis cs:4,0.979932985564595)
--(axis cs:3,0.979642883861932)
--(axis cs:2,0.966454952510589)
--(axis cs:1,0.953295697386423)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.976848125457764)
--(axis cs:1,0.986456036567688)
--(axis cs:2,0.988981068134308)
--(axis cs:3,0.992213249206543)
--(axis cs:4,0.991635799407959)
--(axis cs:5,0.991742670536041)
--(axis cs:6,0.992980241775513)
--(axis cs:7,0.994612276554108)
--(axis cs:7,0.993073880672455)
--(axis cs:7,0.993073880672455)
--(axis cs:6,0.992027640342712)
--(axis cs:5,0.990043103694916)
--(axis cs:4,0.989341855049133)
--(axis cs:3,0.989036798477173)
--(axis cs:2,0.982677280902863)
--(axis cs:1,0.976848125457764)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.9549768
2 0.97209068
3 0.97568476
4 0.9782106
5 0.97989272
6 0.9797938
7 0.98599772
};
%\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.95831848
2 0.97871692
3 0.9847408
4 0.98821304
5 0.98834976
6 0.99182284
7 0.99344708
};%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.96159444
2 0.97817764
3 0.98362928
4 0.98370084
5 0.98153524
6 0.98436924
7 0.98755784
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.981652081012726
2 0.985829174518585
3 0.990625023841858
4 0.990488827228546
5 0.990892887115479
6 0.992503941059113
7 0.993843078613281
};%\addlegendentry{Ours}




==> figures/acc_over_memory_size_100iters_new/PermutedMNIST_acc_over_memory.tex <==
\nextgroupplot[title=Permuted MNIST,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=90},
xticklabels={90,270,450,900,2250},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ylabel={ACC (\%)},
ymin=0.695,%0.637838739156723, 
ymax=0.93909129061632,
ytick style={color=black},
ytick={0.60,0.65,0.7,0.75,0.8,0.85,0.9,0.95},
yticklabels={60,65,70,75,80,85,90,95}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.715730226321196)
--(axis cs:1,0.736885773678804)
--(axis cs:2,0.827973539580458)
--(axis cs:3,0.861050780378148)
--(axis cs:4,0.890440219509845)
--(axis cs:5,0.913933024403524)
--(axis cs:5,0.904794975596476)
--(axis cs:5,0.904794975596476)
--(axis cs:4,0.869939780490155)
--(axis cs:3,0.833253219621852)
--(axis cs:2,0.812214460419542)
--(axis cs:1,0.715730226321196)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.703322259916344)
--(axis cs:1,0.726421740083656)
--(axis cs:2,0.813376771868685)
--(axis cs:3,0.855015954553463)
--(axis cs:4,0.884852627163868)
--(axis cs:5,0.912982539743805)
--(axis cs:5,0.908409460256195)
--(axis cs:5,0.908409460256195)
--(axis cs:4,0.875559372836131)
--(axis cs:3,0.832572045446536)
--(axis cs:2,0.800187228131315)
--(axis cs:1,0.703322259916344)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.738538401173349)
--(axis cs:1,0.771401598826651)
--(axis cs:2,0.798919804972782)
--(axis cs:3,0.839665791039941)
--(axis cs:4,0.835268339924516)
--(axis cs:5,0.850651036649128)
--(axis cs:5,0.774932963350872)
--(axis cs:5,0.774932963350872)
--(axis cs:4,0.770147660075484)
--(axis cs:3,0.793590208960059)
--(axis cs:2,0.767396195027218)
--(axis cs:1,0.738538401173349)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.709841430187225)
--(axis cs:1,0.723326504230499)
--(axis cs:2,0.824357867240906)
--(axis cs:3,0.859517455101013)
--(axis cs:4,0.893725514411926)
--(axis cs:5,0.927864193916321)
--(axis cs:5,0.921083688735962)
--(axis cs:5,0.921083688735962)
--(axis cs:4,0.88515043258667)
--(axis cs:3,0.851162552833557)
--(axis cs:2,0.817286252975464)
--(axis cs:1,0.709841430187225)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.726308
2 0.820094
3 0.847152
4 0.88019
5 0.909364
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.714872
2 0.806782
3 0.843794
4 0.880206
5 0.910696
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.75497
2 0.783158
3 0.816628
4 0.802708
5 0.812792
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.716583967208862
2 0.820822060108185
3 0.855340003967285
4 0.889437973499298
5 0.924473941326141
};
%\addlegendentry{Ours}


==> figures/acc_over_memory_size_100iters_new/miniImagenet_acc_over_memory.tex <==

\nextgroupplot[title=Split miniImagenet,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.525, 0.575, 0.625, 0.675},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=90},
xticklabels={95,285,475,950,1900},
y grid style={white!69.0196078431373!black},
ymajorgrids, yminorgrids,
%ylabel={ACC},
ymin=0.485468408535527, ymax=0.656408178377217,
ytick style={color=black},
ytick={0.5,0.55,0.6,0.65,0.70},
yticklabels={50,55,60,65,70}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.511239936034333)
--(axis cs:1,0.530000063965667)
--(axis cs:2,0.589402344070757)
--(axis cs:3,0.607880865354614)
--(axis cs:4,0.627174196127067)
--(axis cs:5,0.636374896060481)
--(axis cs:5,0.622665103939519)
--(axis cs:5,0.622665103939519)
--(axis cs:4,0.610225803872933)
--(axis cs:3,0.582919134645386)
--(axis cs:2,0.567557655929243)
--(axis cs:1,0.511239936034333)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.493238398073785)
--(axis cs:1,0.533441601926215)
--(axis cs:2,0.57011855059778)
--(axis cs:3,0.605819593487538)
--(axis cs:4,0.614540951326373)
--(axis cs:5,0.630535426185857)
--(axis cs:5,0.616984573814143)
--(axis cs:5,0.616984573814143)
--(axis cs:4,0.595619048673627)
--(axis cs:3,0.586140406512462)
--(axis cs:2,0.55356144940222)
--(axis cs:1,0.493238398073785)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.492947858361007)
--(axis cs:1,0.520172141638993)
--(axis cs:2,0.555463345135852)
--(axis cs:3,0.547130468985637)
--(axis cs:4,0.556312161267811)
--(axis cs:5,0.595653887589556)
--(axis cs:5,0.532706112410444)
--(axis cs:5,0.532706112410444)
--(axis cs:4,0.463447838732189)
--(axis cs:3,0.455229531014363)
--(axis cs:2,0.511216654864149)
--(axis cs:1,0.492947858361007)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.533491373062134)
--(axis cs:1,0.538228631019592)
--(axis cs:2,0.57997077703476)
--(axis cs:3,0.604763567447662)
--(axis cs:4,0.625060558319092)
--(axis cs:5,0.648638188838959)
--(axis cs:5,0.627881824970245)
--(axis cs:5,0.627881824970245)
--(axis cs:4,0.611339330673218)
--(axis cs:3,0.595156371593475)
--(axis cs:2,0.578189194202423)
--(axis cs:1,0.533491373062134)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.52062
2 0.57848
3 0.5954
4 0.6187
5 0.62952
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.51334
2 0.56184
3 0.59598
4 0.60508
5 0.62376
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.50656
2 0.53334
3 0.50118
4 0.50988
5 0.56418
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.535860002040863
2 0.579079985618591
3 0.599959969520569
4 0.618199944496155
5 0.638260006904602
};
%\addlegendentry{RS-MCTS}





==> figures/acc_over_memory_size_100iters_new/notMNIST_acc_over_memory.tex <==
\nextgroupplot[title=Split notMNIST,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.91, 0.93, 0.95, 0.97},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
%xlabel={Memory size \(\displaystyle M\)},
xmin=0.7, xmax=7.3,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=90},
xticklabels={8,24,80,120,200,400,800},
y grid style={white!69.0196078431373!black},
ymajorgrids,
yminorgrids,
%ylabel={ACC},
ymin=0.899, ymax=0.968037298370892,
ytick style={color=black},
ytick={0.9,0.92,0.94,0.96,0.98},
yticklabels={90, 92, 94, 96, 98}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.896013207305508)
--(axis cs:1,0.931135192694492)
--(axis cs:2,0.938159623242489)
--(axis cs:3,0.950881648994029)
--(axis cs:4,0.959366722972026)
--(axis cs:5,0.953366381554805)
--(axis cs:6,0.957957912748783)
--(axis cs:7,0.956996714641506)
--(axis cs:7,0.942492645358494)
--(axis cs:7,0.942492645358494)
--(axis cs:6,0.935719447251217)
--(axis cs:5,0.925448018445195)
--(axis cs:4,0.938790317027974)
--(axis cs:3,0.931924351005971)
--(axis cs:2,0.908068296757511)
--(axis cs:1,0.896013207305508)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.905642837956127)
--(axis cs:1,0.936302282043873)
--(axis cs:2,0.945930444061739)
--(axis cs:3,0.952986088925952)
--(axis cs:4,0.959824157530047)
--(axis cs:5,0.952829054017519)
--(axis cs:6,0.959656752670672)
--(axis cs:7,0.962564882794123)
--(axis cs:7,0.947773837205876)
--(axis cs:7,0.947773837205876)
--(axis cs:6,0.948538687329328)
--(axis cs:5,0.942894385982481)
--(axis cs:4,0.946525122469953)
--(axis cs:3,0.939538551074048)
--(axis cs:2,0.917796675938261)
--(axis cs:1,0.905642837956127)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.92575112968193)
--(axis cs:1,0.94785415031807)
--(axis cs:2,0.955205714329457)
--(axis cs:3,0.958007719572493)
--(axis cs:4,0.952085855254064)
--(axis cs:5,0.955086757682649)
--(axis cs:6,0.947191690371997)
--(axis cs:7,0.964993528242304)
--(axis cs:7,0.936188951757696)
--(axis cs:7,0.936188951757696)
--(axis cs:6,0.909628229628003)
--(axis cs:5,0.922580682317351)
--(axis cs:4,0.916396464745937)
--(axis cs:3,0.906849720427507)
--(axis cs:2,0.904118125670543)
--(axis cs:1,0.92575112968193)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.939071178436279)
--(axis cs:1,0.951526403427124)
--(axis cs:2,0.958871364593506)
--(axis cs:3,0.954144775867462)
--(axis cs:4,0.952358484268188)
--(axis cs:5,0.95714259147644)
--(axis cs:6,0.956836819648743)
--(axis cs:7,0.9615877866745)
--(axis cs:7,0.9475919008255)
--(axis cs:7,0.9475919008255)
--(axis cs:6,0.94806444644928)
--(axis cs:5,0.94659161567688)
--(axis cs:4,0.93076229095459)
--(axis cs:3,0.942625343799591)
--(axis cs:2,0.945715665817261)
--(axis cs:1,0.939071178436279)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.9135742
2 0.92311396
3 0.941403
4 0.94907852
5 0.9394072
6 0.94683868
7 0.94974468
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.92097256
2 0.93186356
3 0.94626232
4 0.95317464
5 0.94786172
6 0.95409772
7 0.95516936
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.93680264
2 0.92966192
3 0.93242872
4 0.93424116
5 0.93883372
6 0.92840996
7 0.95059124
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.945298790931702
2 0.952293515205383
3 0.948385059833527
4 0.941560387611389
5 0.95186710357666
6 0.952450633049011
7 0.95458984375
};
%\addlegendentry{RS-MCTS}



==> figures/acc_over_memory_size_100iters_old/CIFAR100_acc_over_memory.tex <==

\nextgroupplot[title=Split CIFAR-100,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={95,285,475,950,1900},
y grid style={white!69.0196078431373!black},
ymajorgrids,
%ylabel={ACC},
ymin=0.495, ymax=0.810957793848251,
ytick style={color=black},
ytick={0.5, 0.55, 0.6,0.65,0.7,0.75,0.8,0.85},
yticklabels={50, 55, 60, 65, 70, 75, 80, 85}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.567187964916229)
--(axis cs:1,0.595052063465118)
--(axis cs:2,0.683687448501587)
--(axis cs:3,0.721232891082764)
--(axis cs:4,0.759949862957001)
--(axis cs:5,0.789501786231995)
--(axis cs:5,0.782858371734619)
--(axis cs:5,0.782858371734619)
--(axis cs:4,0.748370110988617)
--(axis cs:3,0.711007118225098)
--(axis cs:2,0.667912483215332)
--(axis cs:1,0.567187964916229)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.54420843806795)
--(axis cs:1,0.55951156193205)
--(axis cs:2,0.660018780412226)
--(axis cs:3,0.701282341220295)
--(axis cs:4,0.74849294674193)
--(axis cs:5,0.780335209714517)
--(axis cs:5,0.772824790285483)
--(axis cs:5,0.772824790285483)
--(axis cs:4,0.73630705325807)
--(axis cs:3,0.686757658779705)
--(axis cs:2,0.640341219587774)
--(axis cs:1,0.54420843806795)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.499704018706963)
--(axis cs:1,0.577535981293037)
--(axis cs:2,0.631322030526373)
--(axis cs:3,0.68081333911034)
--(axis cs:4,0.714779020310597)
--(axis cs:5,0.698210881385584)
--(axis cs:5,0.575789118614416)
--(axis cs:5,0.575789118614416)
--(axis cs:4,0.604540979689403)
--(axis cs:3,0.61926666088966)
--(axis cs:2,0.573797969473627)
--(axis cs:1,0.499704018706963)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.594093382358551)
--(axis cs:1,0.615146577358246)
--(axis cs:2,0.694118440151215)
--(axis cs:3,0.734759986400604)
--(axis cs:4,0.772708475589752)
--(axis cs:5,0.798255443572998)
--(axis cs:5,0.786504507064819)
--(axis cs:5,0.786504507064819)
--(axis cs:4,0.760211646556854)
--(axis cs:3,0.723879992961884)
--(axis cs:2,0.682881414890289)
--(axis cs:1,0.594093382358551)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.581120014190674
2 0.675799965858459
3 0.716120004653931
4 0.754159986972809
5 0.786180078983307
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.55186
2 0.65018
3 0.69402
4 0.7424
5 0.77658
};

\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.53862
2 0.60256
3 0.65004
4 0.65966
5 0.637
};

\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.604619979858398
2 0.688499927520752
3 0.729319989681244
4 0.766460061073303
5 0.792379975318909
};




==> figures/acc_over_memory_size_100iters_old/FashionMNIST_acc_over_memory.tex <==

\nextgroupplot[title=Split FashionMNIST,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.89, 0.91, 0.93, 0.95, 0.97, 0.99},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
%xlabel={Memory size \(\displaystyle M\)},
xmin=0.7, xmax=7.3,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=90},
xticklabels={8,24,80,120,200,400,800},
y grid style={white!69.0196078431373!black},
ymajorgrids,
yminorgrids,
%ylabel={ACC},
ymin=0.899,%0.891766529814355,
ymax=0.996494715797058,
ytick style={color=black},
ytick={0.88,0.9,0.92,0.94,0.96,0.98,1},
yticklabels={88, 90, 92, 94, 96, 98, 100}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.96419358253479)
--(axis cs:1,0.976246356964111)
--(axis cs:2,0.984048008918762)
--(axis cs:3,0.98274040222168)
--(axis cs:4,0.982234418392181)
--(axis cs:5,0.985867142677307)
--(axis cs:6,0.985980749130249)
--(axis cs:7,0.988571465015411)
--(axis cs:7,0.980668723583221)
--(axis cs:7,0.980668723583221)
--(axis cs:6,0.972739219665527)
--(axis cs:5,0.975212812423706)
--(axis cs:4,0.954325616359711)
--(axis cs:3,0.976219773292542)
--(axis cs:2,0.962551951408386)
--(axis cs:1,0.96419358253479)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.965724160568608)
--(axis cs:1,0.979275839431391)
--(axis cs:2,0.983843648420532)
--(axis cs:3,0.987767732323772)
--(axis cs:4,0.988072744085454)
--(axis cs:5,0.988506841180757)
--(axis cs:6,0.989178836422143)
--(axis cs:7,0.990307375485654)
--(axis cs:7,0.989052624514346)
--(axis cs:7,0.989052624514346)
--(axis cs:6,0.987461163577857)
--(axis cs:5,0.983413158819243)
--(axis cs:4,0.982567255914546)
--(axis cs:3,0.970792267676228)
--(axis cs:2,0.972876351579468)
--(axis cs:1,0.965724160568608)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.955000050761585)
--(axis cs:1,0.970759949238415)
--(axis cs:2,0.98603178628668)
--(axis cs:3,0.981832320290786)
--(axis cs:4,0.983967730086771)
--(axis cs:5,0.978253058795492)
--(axis cs:6,0.991734343706935)
--(axis cs:7,0.969833098095523)
--(axis cs:7,0.896526901904478)
--(axis cs:7,0.896526901904478)
--(axis cs:6,0.916425656293065)
--(axis cs:5,0.938266941204508)
--(axis cs:4,0.921192269913229)
--(axis cs:3,0.942567679709214)
--(axis cs:2,0.92920821371332)
--(axis cs:1,0.955000050761585)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.982129275798798)
--(axis cs:1,0.984390676021576)
--(axis cs:2,0.987218379974365)
--(axis cs:3,0.988464534282684)
--(axis cs:4,0.989360094070435)
--(axis cs:5,0.989464402198792)
--(axis cs:6,0.989146828651428)
--(axis cs:7,0.990860760211945)
--(axis cs:7,0.988419115543365)
--(axis cs:7,0.988419115543365)
--(axis cs:6,0.98689329624176)
--(axis cs:5,0.987175583839417)
--(axis cs:4,0.985639929771423)
--(axis cs:3,0.983615458011627)
--(axis cs:2,0.982341647148132)
--(axis cs:1,0.982129275798798)
--cycle;
\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.970219969749451
2 0.973299980163574
3 0.979480087757111
4 0.968280017375946
5 0.980539977550507
6 0.979359984397888
7 0.984620094299316
};
%\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.9725
2 0.97836
3 0.97928
4 0.98532
5 0.98596
6 0.98832
7 0.98968
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.96288
2 0.95762
3 0.9622
4 0.95258
5 0.95826
6 0.95408
7 0.93318
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.983259975910187
2 0.984780013561249
3 0.986039996147156
4 0.987500011920929
5 0.988319993019104
6 0.988020062446594
7 0.989639937877655
};
%\addlegendentry{Ours}



==> figures/acc_over_memory_size_100iters_old/MNIST_acc_over_memory.tex <==
\nextgroupplot[title=Split MNIST,
height=\figheight,
legend cell align={left},
%legend style={
%  nodes={scale=1.0},%=0.95},%{scale=0.9},
%  fill opacity=0.8,
%  draw opacity=1,
%  text opacity=1,
%  at={(3.90,-0.15)}, %{(3.70,-0.30)},   %{(3.72,0.13)},
%  anchor=south west,
%  draw=white!80!black
%},
legend columns=-1,
legend style={
  nodes={scale=0.85},%=0.95},%{scale=0.9},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,1.28)}, %{(3.70,-0.30)},   %{(3.72,0.13)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
%xlabel={Memory size \(\displaystyle M\)},
xmin=0.7, xmax=7.3,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=90},
xticklabels={8,24,80,120,200,400,800},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ylabel={ACC (\%)},
ymin=0.939, ymax=0.997729043511215,
ytick style={color=black},
ytick={0.92,0.93,0.94,0.95,0.96,0.97,0.98,0.99,1},
yticklabels={92,93,94,95,96,97,98,99,100}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.92504620552063)
--(axis cs:1,0.981783270835876)
--(axis cs:2,0.981537520885468)
--(axis cs:3,0.988991677761078)
--(axis cs:4,0.986135482788086)
--(axis cs:5,0.991755723953247)
--(axis cs:6,0.989374697208405)
--(axis cs:7,0.994002878665924)
--(axis cs:7,0.976767957210541)
--(axis cs:7,0.976767957210541)
--(axis cs:6,0.979170620441437)
--(axis cs:5,0.964531421661377)
--(axis cs:4,0.978874921798706)
--(axis cs:3,0.979120314121246)
--(axis cs:2,0.937642157077789)
--(axis cs:1,0.92504620552063)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.946015386753438)
--(axis cs:1,0.970621573246562)
--(axis cs:2,0.984533286206628)
--(axis cs:3,0.988692537329328)
--(axis cs:4,0.990023216819651)
--(axis cs:5,0.990669279851693)
--(axis cs:6,0.992800317892538)
--(axis cs:7,0.994021984494329)
--(axis cs:7,0.992872175505671)
--(axis cs:7,0.992872175505671)
--(axis cs:6,0.990845362107462)
--(axis cs:5,0.986030240148307)
--(axis cs:4,0.986402863180349)
--(axis cs:3,0.980789062670673)
--(axis cs:2,0.972900553793372)
--(axis cs:1,0.946015386753438)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.953295697386423)
--(axis cs:1,0.969893182613577)
--(axis cs:2,0.989900327489411)
--(axis cs:3,0.987615676138068)
--(axis cs:4,0.987468694435405)
--(axis cs:5,0.987904186526891)
--(axis cs:6,0.990390603540462)
--(axis cs:7,0.991611458769248)
--(axis cs:7,0.983504221230752)
--(axis cs:7,0.983504221230752)
--(axis cs:6,0.978347876459538)
--(axis cs:5,0.975166293473109)
--(axis cs:4,0.979932985564595)
--(axis cs:3,0.979642883861932)
--(axis cs:2,0.966454952510589)
--(axis cs:1,0.953295697386423)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.976848125457764)
--(axis cs:1,0.986456036567688)
--(axis cs:2,0.988981068134308)
--(axis cs:3,0.992213249206543)
--(axis cs:4,0.991635799407959)
--(axis cs:5,0.991742670536041)
--(axis cs:6,0.992980241775513)
--(axis cs:7,0.994612276554108)
--(axis cs:7,0.993073880672455)
--(axis cs:7,0.993073880672455)
--(axis cs:6,0.992027640342712)
--(axis cs:5,0.990043103694916)
--(axis cs:4,0.989341855049133)
--(axis cs:3,0.989036798477173)
--(axis cs:2,0.982677280902863)
--(axis cs:1,0.976848125457764)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.953414738178253
2 0.959589838981628
3 0.984055995941162
4 0.982505202293396
5 0.978143572807312
6 0.984272658824921
7 0.985385417938232
};
\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.95831848
2 0.97871692
3 0.9847408
4 0.98821304
5 0.98834976
6 0.99182284
7 0.99344708
};\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.96159444
2 0.97817764
3 0.98362928
4 0.98370084
5 0.98153524
6 0.98436924
7 0.98755784
};
\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.981652081012726
2 0.985829174518585
3 0.990625023841858
4 0.990488827228546
5 0.990892887115479
6 0.992503941059113
7 0.993843078613281
};\addlegendentry{Ours}




==> figures/acc_over_memory_size_100iters_old/PermutedMNIST_acc_over_memory.tex <==
\nextgroupplot[title=Permuted MNIST,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={90,270,450,900,2250},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ylabel={ACC (\%)},
ymin=0.637838739156723, ymax=0.93909129061632,
ytick style={color=black},
ytick={0.60,0.65,0.7,0.75,0.8,0.85,0.9,0.95},
yticklabels={60,65,70,75,80,85,90,95}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.651649475097656)
--(axis cs:1,0.679890394210815)
--(axis cs:2,0.806510269641876)
--(axis cs:3,0.825519323348999)
--(axis cs:4,0.878083646297455)
--(axis cs:5,0.909908771514893)
--(axis cs:5,0.906343221664429)
--(axis cs:5,0.906343221664429)
--(axis cs:4,0.867364227771759)
--(axis cs:3,0.817520618438721)
--(axis cs:2,0.77967768907547)
--(axis cs:1,0.651649475097656)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.703322259916344)
--(axis cs:1,0.726421740083656)
--(axis cs:2,0.813376771868685)
--(axis cs:3,0.855015954553463)
--(axis cs:4,0.884852627163868)
--(axis cs:5,0.912982539743805)
--(axis cs:5,0.908409460256195)
--(axis cs:5,0.908409460256195)
--(axis cs:4,0.875559372836131)
--(axis cs:3,0.832572045446536)
--(axis cs:2,0.800187228131315)
--(axis cs:1,0.703322259916344)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.738538401173349)
--(axis cs:1,0.771401598826651)
--(axis cs:2,0.798919804972782)
--(axis cs:3,0.839665791039941)
--(axis cs:4,0.835268339924516)
--(axis cs:5,0.850651036649128)
--(axis cs:5,0.774932963350872)
--(axis cs:5,0.774932963350872)
--(axis cs:4,0.770147660075484)
--(axis cs:3,0.793590208960059)
--(axis cs:2,0.767396195027218)
--(axis cs:1,0.738538401173349)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.709841430187225)
--(axis cs:1,0.723326504230499)
--(axis cs:2,0.824357867240906)
--(axis cs:3,0.859517455101013)
--(axis cs:4,0.893725514411926)
--(axis cs:5,0.927864193916321)
--(axis cs:5,0.921083688735962)
--(axis cs:5,0.921083688735962)
--(axis cs:4,0.88515043258667)
--(axis cs:3,0.851162552833557)
--(axis cs:2,0.817286252975464)
--(axis cs:1,0.709841430187225)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.665769934654236
2 0.793093979358673
3 0.82151997089386
4 0.872723937034607
5 0.908125996589661
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.714872
2 0.806782
3 0.843794
4 0.880206
5 0.910696
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.75497
2 0.783158
3 0.816628
4 0.802708
5 0.812792
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.716583967208862
2 0.820822060108185
3 0.855340003967285
4 0.889437973499298
5 0.924473941326141
};
%\addlegendentry{Ours}


==> figures/acc_over_memory_size_100iters_old/acc_over_memory_size_groupplot.tex <==



\pgfplotsset{every axis title/.append style={at={(0.5,0.80)}}} %{at={(0.5,0.84)}}}
\pgfplotsset{every tick label/.append style={font=\tiny}}
\pgfplotsset{every major tick/.append style={major tick length=2pt}}
\pgfplotsset{every minor tick/.append style={minor tick length=1pt}}
\pgfplotsset{every axis x label/.append style={at={(0.5,-0.27)}}}
\pgfplotsset{every axis y label/.append style={at={(-0.20,0.5)}}}
\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{groupplot}[group style={group size= 3 by 2, horizontal sep=0.9cm, vertical sep=0.9cm}]

\input{figures/acc_over_memory_size_100iters/MNIST_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/FashionMNIST_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/notMNIST_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/PermutedMNIST_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/CIFAR100_acc_over_memory}

\input{figures/acc_over_memory_size_100iters/miniImagenet_acc_over_memory}

\end{groupplot}

\end{tikzpicture}

==> figures/acc_over_memory_size_100iters_old/miniImagenet_acc_over_memory.tex <==

\nextgroupplot[title=Split miniImagenet,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.525, 0.575, 0.625, 0.675},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={95,285,475,950,1900},
y grid style={white!69.0196078431373!black},
ymajorgrids, yminorgrids,
%ylabel={ACC},
ymin=0.485468408535527, ymax=0.656408178377217,
ytick style={color=black},
ytick={0.5,0.55,0.6,0.65,0.70},
yticklabels={50,55,60,65,70}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.510739743709564)
--(axis cs:1,0.526020228862762)
--(axis cs:2,0.560024738311768)
--(axis cs:3,0.586868524551392)
--(axis cs:4,0.607182204723358)
--(axis cs:5,0.620157301425934)
--(axis cs:5,0.612762629985809)
--(axis cs:5,0.612762629985809)
--(axis cs:4,0.584657728672028)
--(axis cs:3,0.566691517829895)
--(axis cs:2,0.545615077018738)
--(axis cs:1,0.510739743709564)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.493238398073785)
--(axis cs:1,0.533441601926215)
--(axis cs:2,0.57011855059778)
--(axis cs:3,0.605819593487538)
--(axis cs:4,0.614540951326373)
--(axis cs:5,0.630535426185857)
--(axis cs:5,0.616984573814143)
--(axis cs:5,0.616984573814143)
--(axis cs:4,0.595619048673627)
--(axis cs:3,0.586140406512462)
--(axis cs:2,0.55356144940222)
--(axis cs:1,0.493238398073785)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.492947858361007)
--(axis cs:1,0.520172141638993)
--(axis cs:2,0.555463345135852)
--(axis cs:3,0.547130468985637)
--(axis cs:4,0.556312161267811)
--(axis cs:5,0.595653887589556)
--(axis cs:5,0.532706112410444)
--(axis cs:5,0.532706112410444)
--(axis cs:4,0.463447838732189)
--(axis cs:3,0.455229531014363)
--(axis cs:2,0.511216654864149)
--(axis cs:1,0.492947858361007)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.533491373062134)
--(axis cs:1,0.538228631019592)
--(axis cs:2,0.57997077703476)
--(axis cs:3,0.604763567447662)
--(axis cs:4,0.625060558319092)
--(axis cs:5,0.648638188838959)
--(axis cs:5,0.627881824970245)
--(axis cs:5,0.627881824970245)
--(axis cs:4,0.611339330673218)
--(axis cs:3,0.595156371593475)
--(axis cs:2,0.578189194202423)
--(axis cs:1,0.533491373062134)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.518379986286163
2 0.552819907665253
3 0.576780021190643
4 0.595919966697693
5 0.616459965705872
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.51334
2 0.56184
3 0.59598
4 0.60508
5 0.62376
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.50656
2 0.53334
3 0.50118
4 0.50988
5 0.56418
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.535860002040863
2 0.579079985618591
3 0.599959969520569
4 0.618199944496155
5 0.638260006904602
};
%\addlegendentry{RS-MCTS}





==> figures/acc_over_memory_size_100iters_old/notMNIST_acc_over_memory.tex <==
\nextgroupplot[title=Split notMNIST,
height=\figheight,
legend cell align={left},
legend style={
  nodes={scale=0.7},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.48,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.91, 0.93, 0.95, 0.97},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
%xlabel={Memory size \(\displaystyle M\)},
xmin=0.7, xmax=7.3,
xtick style={color=black},
xtick={1,2,3,4,5,6,7},
xticklabel style={rotate=90},
xticklabels={8,24,80,120,200,400,800},
y grid style={white!69.0196078431373!black},
ymajorgrids,
yminorgrids,
%ylabel={ACC},
ymin=0.899, ymax=0.968037298370892,
ytick style={color=black},
ytick={0.9,0.92,0.94,0.96,0.98},
yticklabels={90, 92, 94, 96, 98}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.898027122020721)
--(axis cs:1,0.932646334171295)
--(axis cs:2,0.949522912502289)
--(axis cs:3,0.941804111003876)
--(axis cs:4,0.945932507514954)
--(axis cs:5,0.944690823554993)
--(axis cs:6,0.958006739616394)
--(axis cs:7,0.963123440742493)
--(axis cs:7,0.937735080718994)
--(axis cs:7,0.937735080718994)
--(axis cs:6,0.941412806510925)
--(axis cs:5,0.925552010536194)
--(axis cs:4,0.917471051216125)
--(axis cs:3,0.924349844455719)
--(axis cs:2,0.907234847545624)
--(axis cs:1,0.898027122020721)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.905642837956127)
--(axis cs:1,0.936302282043873)
--(axis cs:2,0.945930444061739)
--(axis cs:3,0.952986088925952)
--(axis cs:4,0.959824157530047)
--(axis cs:5,0.952829054017519)
--(axis cs:6,0.959656752670672)
--(axis cs:7,0.962564882794123)
--(axis cs:7,0.947773837205876)
--(axis cs:7,0.947773837205876)
--(axis cs:6,0.948538687329328)
--(axis cs:5,0.942894385982481)
--(axis cs:4,0.946525122469953)
--(axis cs:3,0.939538551074048)
--(axis cs:2,0.917796675938261)
--(axis cs:1,0.905642837956127)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.92575112968193)
--(axis cs:1,0.94785415031807)
--(axis cs:2,0.955205714329457)
--(axis cs:3,0.958007719572493)
--(axis cs:4,0.952085855254064)
--(axis cs:5,0.955086757682649)
--(axis cs:6,0.947191690371997)
--(axis cs:7,0.964993528242304)
--(axis cs:7,0.936188951757696)
--(axis cs:7,0.936188951757696)
--(axis cs:6,0.909628229628003)
--(axis cs:5,0.922580682317351)
--(axis cs:4,0.916396464745937)
--(axis cs:3,0.906849720427507)
--(axis cs:2,0.904118125670543)
--(axis cs:1,0.92575112968193)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.939071178436279)
--(axis cs:1,0.951526403427124)
--(axis cs:2,0.958871364593506)
--(axis cs:3,0.954144775867462)
--(axis cs:4,0.952358484268188)
--(axis cs:5,0.95714259147644)
--(axis cs:6,0.956836819648743)
--(axis cs:7,0.9615877866745)
--(axis cs:7,0.9475919008255)
--(axis cs:7,0.9475919008255)
--(axis cs:6,0.94806444644928)
--(axis cs:5,0.94659161567688)
--(axis cs:4,0.93076229095459)
--(axis cs:3,0.942625343799591)
--(axis cs:2,0.945715665817261)
--(axis cs:1,0.939071178436279)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.915336728096008
2 0.928378880023956
3 0.933076977729797
4 0.93170177936554
5 0.935121417045593
6 0.94970977306366
7 0.950429260730743
};
%\addlegendentry{Random}

\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.92097256
2 0.93186356
3 0.94626232
4 0.95317464
5 0.94786172
6 0.95409772
7 0.95516936
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.93680264
2 0.92966192
3 0.93242872
4 0.93424116
5 0.93883372
6 0.92840996
7 0.95059124
};
%\addlegendentry{Heuristic}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.945298790931702
2 0.952293515205383
3 0.948385059833527
4 0.941560387611389
5 0.95186710357666
6 0.952450633049011
7 0.95458984375
};
%\addlegendentry{RS-MCTS}



==> figures/bar_plots_acc/accuracies.tex <==
\nextgroupplot[title=Split MNIST,
ybar,
bar width=4pt,
height=\figheight,
legend cell align={left},
legend columns=2, 
legend style={
  nodes={scale=0.8},%=0.85},
  fill opacity=0.8, 
  draw opacity=1, 
  text opacity=1, 
  at={(2.5,1)}, 
  draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorticks=false,
xmin=0, xmax=2,
xtick style={color=black},
%xtick={-1,0,1,2,3,4,5,6},
y grid style={white!69.0196078431373!black},
ylabel={ACC (\%)},
ymajorgrids,
ymin=85, ymax=101,
ytick style={color=black},
%ytick={80,90,92,94,96,98,100}
]
\addplot [draw=black, fill=color0, error bars/.cd, y dir=both, y explicit,  
] coordinates {
    (1.00,99.75) +- (0,0.06)
};
\addlegendentry{Joint}

\addplot [draw=black, fill=purple, error bars/.cd, y dir=both, y explicit,
] coordinates {
    (1.05,98.28) +- (0,0.49)
};
\addlegendentry{BFS}

\addplot [draw=black, fill=color1, error bars/.cd, y dir=both, y explicit,
] coordinates {
    (1.10,94.91) +- (0,2.52)
};
\addlegendentry{Random}

\addplot [draw=black, fill=color2, error bars/.cd, y dir=both, y explicit, 
] coordinates {
    (1.15,94.02) +- (0,4.25)
};
\addlegendentry{ETS}

\addplot [draw=black, fill=color3, error bars/.cd, y dir=both, y explicit, 
] coordinates {
    (1.20,96.02) +- (0,2.32)
};
\addlegendentry{Heur-GD}

\addplot [draw=black, fill=color4, error bars/.cd, y dir=both, y explicit, 
] coordinates {
    (1.25,95.72) +- (0,2.14)
};
\addlegendentry{Heur-LD}

\addplot [draw=black, fill=color5, error bars/.cd, y dir=both, y explicit, 
] coordinates {
    (1.30,96.75) +- (0,1.31)
};
\addlegendentry{Heur-AT}

\addplot [draw=black, fill=color6, error bars/.cd, y dir=both, y explicit, 
] coordinates {
    (1.35,97.93) +- (0,0.56)
};
\addlegendentry{MCTS}

\begin{comment}
\addplot [draw=black, fill=color0] coordinates {
(0.3,94.906244)
};\addlegendentry{Random}
\path [draw=black, line width=1.0pt]
(axis cs:0.3,92.3846798070943)
--(axis cs:0.3,97.4278081929057);
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
0.3 92.3846798070943
};
%\addlegendentry{MCTS}
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
0.3 97.4278081929057
};
%\addlegendentry{MCTS}
%\draw[draw=none,fill=color0,line width=13.0pt] (axis cs:0.1,0) rectangle (axis cs:0.5,94.906244);
%\addlegendimage{ybar,ybar legend,draw=none,fill=color0,line width=1pt}
%\addlegendentry{Random}

\addplot [draw=black, fill=color1] coordinates {
(1.3,94.021292)
};\addlegendentry{ETS}
\path [draw=black, line width=1.0pt]
(axis cs:1.3,89.7697592101916)
--(axis cs:1.3,98.2728247898084);
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
1.3 89.7697592101916
};
%\addlegendentry{MCTS}
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
1.3 98.2728247898084
};
%\addlegendentry{MCTS}
%\draw[draw=none,fill=color1,line width=13.0pt] (axis cs:1.1,0) rectangle (axis cs:1.5,94.021292);
%\addlegendimage{ybar,ybar legend,draw=none,fill=color1,line width=1pt}
%\addlegendentry{ETS}


\draw[draw=none,fill=color2,line width=13.0pt] (axis cs:2.1,0) rectangle (axis cs:2.5,96.024116);
\addlegendimage{ybar,ybar legend,draw=none,fill=color2,line width=1pt}
\addlegendentry{Heuristic GD}

\draw[draw=none,fill=color3,line width=13.0pt] (axis cs:3.1,0) rectangle (axis cs:3.5,95.722052);
\addlegendimage{ybar,ybar legend,draw=none,fill=color3,line width=1pt}
\addlegendentry{Heuristic LD}

\draw[draw=none,fill=color4,line width=13.0pt] (axis cs:4.1,0) rectangle (axis cs:4.5,96.753928);
\addlegendimage{ybar,ybar legend,draw=none,fill=color4,line width=1pt}
\addlegendentry{Heuristic AT}

\draw[draw=none,fill=color5,line width=13.0pt] (axis cs:5.1,0) rectangle (axis cs:5.5,97.9289412498474);
%\addlegendimage{ybar,ybar legend,draw=none,fill=color5,line width=1pt}
\addlegendentry{MCTS}





\path [draw=black, line width=1.0pt]
(axis cs:2.3,93.7059341570067)
--(axis cs:2.3,98.3422978429933);

\path [draw=black, line width=1.0pt]
(axis cs:3.3,93.5830088544192)
--(axis cs:3.3,97.8610951455807);

\path [draw=black, line width=1.0pt]
(axis cs:4.3,95.4451227810251)
--(axis cs:4.3,98.0627332189749);

\path [draw=black, line width=1.0pt]
(axis cs:5.3,97.3717656452209)
--(axis cs:5.3,98.4861168544739);



\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
2.3 93.7059341570067
};
%\addlegendentry{MCTS}
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
2.3 98.3422978429933
};
%\addlegendentry{MCTS}
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
3.3 93.5830088544192
};
%\addlegendentry{MCTS}
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
3.3 97.8610951455807
};
%\addlegendentry{MCTS}
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
4.3 95.4451227810251
};
%\addlegendentry{MCTS}
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
4.3 98.0627332189749
};
%\addlegendentry{MCTS}
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
5.3 97.3717656452209
};
%\addlegendentry{MCTS}
\addplot [line width=1.0pt, black, mark=-, mark size=1, mark options={solid}, only marks]
table {%
5.3 98.4861168544739
};
%\addlegendentry{MCTS}
\end{comment}

==> figures/bar_plots_acc/forgetting.tex <==
\nextgroupplot[title=Split MNIST,
height=\figheight,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1,1)}, draw=white!80!black},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmin=-0.17, xmax=5.77,
xtick style={color=black},
xtick={-1,0,1,2,3,4,5,6},
y grid style={white!69.0196078431373!black},
ylabel={BWT (\%)},
ymajorgrids,
ymin=-13.1767426710356, ymax=0,
ytick style={color=black},
ytick={-14,-12,-10,-8,-6,-4,-2,0}
]
\draw[draw=none,fill=color0,line width=1pt] (axis cs:0.1,0) rectangle (axis cs:0.5,-6.12700611352921);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0,line width=1pt}
%\addlegendentry{Random}

\draw[draw=none,fill=color1,line width=1pt] (axis cs:1.1,0) rectangle (axis cs:1.5,-7.22297191619873);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1,line width=1pt}
%\addlegendentry{ETS}

\draw[draw=none,fill=color2,line width=1pt] (axis cs:2.1,0) rectangle (axis cs:2.5,-4.63898360729218);
\addlegendimage{ybar,ybar legend,draw=none,fill=color2,line width=1pt}
%\addlegendentry{Heuristic GD}

\draw[draw=none,fill=color3,line width=1pt] (axis cs:3.1,0) rectangle (axis cs:3.5,-5.01923710107803);
\addlegendimage{ybar,ybar legend,draw=none,fill=color3,line width=1pt}
%\addlegendentry{Heuristic LD}

\draw[draw=none,fill=color4,line width=1pt] (axis cs:4.1,0) rectangle (axis cs:4.5,-3.7369641661644);
\addlegendimage{ybar,ybar legend,draw=none,fill=color4,line width=1pt}
%\addlegendentry{Heuristic AT}

\draw[draw=none,fill=color5,line width=1pt] (axis cs:5.1,0) rectangle (axis cs:5.5,-2.26812243461609);
\addlegendimage{ybar,ybar legend,draw=none,fill=color5,line width=1pt}
%\addlegendentry{MCTS}

\path [draw=black, line width=1.5pt]
(axis cs:0.3,-9.28803807085097)
--(axis cs:0.3,-2.96597415620744);

\path [draw=black, line width=1.5pt]
(axis cs:1.3,-12.5492787343196)
--(axis cs:1.3,-1.89666509807784);

\path [draw=black, line width=1.5pt]
(axis cs:2.3,-7.53998521947844)
--(axis cs:2.3,-1.73798199510592);

\path [draw=black, line width=1.5pt]
(axis cs:3.3,-7.70182533685119)
--(axis cs:3.3,-2.33664886530488);

\path [draw=black, line width=1.5pt]
(axis cs:4.3,-5.38415615448826)
--(axis cs:4.3,-2.08977217784054);

\path [draw=black, line width=1.5pt]
(axis cs:5.3,-2.97618277346155)
--(axis cs:5.3,-1.56006209577063);

\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0.3 -9.28803807085097
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
0.3 -2.96597415620744
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
1.3 -12.5492787343196
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
1.3 -1.89666509807784
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
2.3 -7.53998521947844
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
2.3 -1.73798199510592
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
3.3 -7.70182533685119
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
3.3 -2.33664886530488
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
4.3 -5.38415615448826
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
4.3 -2.08977217784054
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
5.3 -2.97618277346155
};
%%\addlegendentry{MCTS}
\addplot [line width=1.5pt, black, mark=-, mark size=3, mark options={solid}, only marks]
table {%
5.3 -1.56006209577063
};
%%\addlegendentry{MCTS}



==> figures/bar_plots_acc/groupplot.tex <==

\pgfplotsset{compat=1.11,
    /pgfplots/ybar legend/.style={
    /pgfplots/legend image code/.code={%
       \draw[##1,/tikz/.cd,yshift=-0.25em]
        (0cm,0cm) rectangle (3pt,0.8em);},
   },
}
\begin{tikzpicture}
%\tikzstyle{every node}=[font=\scriptsize]
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{groupplot}[group style={group size= 1 by 1, horizontal sep=1.9cm, vertical sep=0.9cm}]

\input{figures/bar_plots_accs/accuracies.tex}

%\input{figures/bar_plots_accs/accuracies.tex}

%\input{figures/bar_plots_accs/forgetting.tex}

%\input{figures/bar_plots_accs/forgetting.tex}

\end{groupplot}

\end{tikzpicture}

==> figures/class_il_scenario/CIFAR100_acc_over_memory.tex <==
\nextgroupplot[title=Split CIFAR-100,
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.025, 0.075, 0.125, 0.175, 0.225},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xmajorgrids,
xlabel={Memory size \(\displaystyle M\)},
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=90},
xticklabels={100,200,400,800,1600},
y grid style={white!69.0196078431373!black},
ymajorgrids, yminorgrids,
ylabel={ACC (\%)},
ymin=0.0369820315859416, ymax=0.186984212534666,
ytick style={color=black},
ytick={0.0,0.05,0.10,0.15,0.20,0.25},
yticklabels={0,5,10,15,20,25}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.0445679784952452)
--(axis cs:1,0.0453120215047548)
--(axis cs:2,0.0536421292893962)
--(axis cs:3,0.073841679435899)
--(axis cs:4,0.111484486208065)
--(axis cs:5,0.162301395207369)
--(axis cs:5,0.148538604792631)
--(axis cs:5,0.148538604792631)
--(axis cs:4,0.101315513791935)
--(axis cs:3,0.068838320564101)
--(axis cs:2,0.0511978707106038)
--(axis cs:1,0.0445679784952452)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.0438003125381563)
--(axis cs:1,0.0463596874618437)
--(axis cs:2,0.051187725463806)
--(axis cs:3,0.0659694979413528)
--(axis cs:4,0.0933042529486208)
--(axis cs:5,0.143101874451005)
--(axis cs:5,0.136698125548995)
--(axis cs:5,0.136698125548995)
--(axis cs:4,0.0892557470513792)
--(axis cs:3,0.0609905020586472)
--(axis cs:2,0.048332274536194)
--(axis cs:1,0.0438003125381563)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.0442478019326001)
--(axis cs:1,0.0467521980673999)
--(axis cs:2,0.053592546295606)
--(axis cs:3,0.0826581724800806)
--(axis cs:4,0.117993399620744)
--(axis cs:5,0.175061735276269)
--(axis cs:5,0.138178264723731)
--(axis cs:5,0.138178264723731)
--(axis cs:4,0.108606600379256)
--(axis cs:3,0.0706218275199194)
--(axis cs:2,0.050487453704394)
--(axis cs:1,0.0442478019326001)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.0451920330524445)
--(axis cs:1,0.0472079664468765)
--(axis cs:2,0.0600229986011982)
--(axis cs:3,0.0851799994707108)
--(axis cs:4,0.122953526675701)
--(axis cs:5,0.180165931582451)
--(axis cs:5,0.171714082360268)
--(axis cs:5,0.171714082360268)
--(axis cs:4,0.118206478655338)
--(axis cs:3,0.080939993262291)
--(axis cs:2,0.0568170063197613)
--(axis cs:1,0.0451920330524445)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.04494
2 0.05242
3 0.07134
4 0.1064
5 0.15542
};
%\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.04508
2 0.04976
3 0.06348
4 0.09128
5 0.1399
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.0455
2 0.05204
3 0.07664
4 0.1133
5 0.15662
};
%\addlegendentry{Heuristic GD}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.0461999997496605
2 0.0584200024604797
3 0.0830599963665009
4 0.12058000266552
5 0.175940006971359
};
%\addlegendentry{RS-MCTS}


==> figures/class_il_scenario/FashionMNIST_acc_over_memory.tex <==
\nextgroupplot[title=Split FashionMNIST,
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={},%{Memory size \(\displaystyle M\)},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=90},
xticklabels={10,20,40,100,200},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ylabel={},%{ACC (\%)},
ymin=0.259424595274879, ymax=0.720812421552797,
ytick style={color=black},
ytick={0.2, 0.3, 0.4, 0.5, 0.6, 0.7},
yticklabels={20,30,40,50,60,70}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.280396769196603)
--(axis cs:1,0.335123230803398)
--(axis cs:2,0.407187817882043)
--(axis cs:3,0.48739351280264)
--(axis cs:4,0.592706736474621)
--(axis cs:5,0.663078371171996)
--(axis cs:5,0.559201628828004)
--(axis cs:5,0.559201628828004)
--(axis cs:4,0.526493263525379)
--(axis cs:3,0.42820648719736)
--(axis cs:2,0.348852182117957)
--(axis cs:1,0.280396769196603)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.283089035628021)
--(axis cs:1,0.330270964371979)
--(axis cs:2,0.403394694538454)
--(axis cs:3,0.46754458659089)
--(axis cs:4,0.602092782062309)
--(axis cs:5,0.672530100400932)
--(axis cs:5,0.657589899599068)
--(axis cs:5,0.657589899599068)
--(axis cs:4,0.583147217937691)
--(axis cs:3,0.44329541340911)
--(axis cs:2,0.371885305461546)
--(axis cs:1,0.283089035628021)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.286364363477931)
--(axis cs:1,0.349795636522069)
--(axis cs:2,0.444960565648486)
--(axis cs:3,0.532675570275331)
--(axis cs:4,0.610988944594497)
--(axis cs:5,0.550032759051677)
--(axis cs:5,0.543687240948323)
--(axis cs:5,0.543687240948323)
--(axis cs:4,0.551771055405503)
--(axis cs:3,0.50080442972467)
--(axis cs:2,0.405359434351514)
--(axis cs:1,0.286364363477931)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.310655891895294)
--(axis cs:1,0.364784121513367)
--(axis cs:2,0.464605748653412)
--(axis cs:3,0.542859613895416)
--(axis cs:4,0.633972704410553)
--(axis cs:5,0.699840247631073)
--(axis cs:5,0.647799789905548)
--(axis cs:5,0.647799789905548)
--(axis cs:4,0.585347354412079)
--(axis cs:3,0.483660370111465)
--(axis cs:2,0.420714259147644)
--(axis cs:1,0.310655891895294)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.30776
2 0.37802
3 0.4578
4 0.5596
5 0.61114
};
%\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.30668
2 0.38764
3 0.45542
4 0.59262
5 0.66506
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.31808
2 0.42516
3 0.51674
4 0.58138
5 0.54686
};
%\addlegendentry{Heuristic GD}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.33772000670433
2 0.442660003900528
3 0.513260006904602
4 0.609660029411316
5 0.673820018768311
};
%\addlegendentry{RS-MCTS}


==> figures/class_il_scenario/MNIST_acc_over_memory.tex <==
% This file was created with tikzplotlib v0.9.12.

\nextgroupplot[title=Split MNIST,
height=\figheight,
legend cell align={left},
legend columns=1,
legend style={
  nodes={scale=0.85},%=0.95},%{scale=0.85},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(2.45,-1.65)}, %{(3.70,-0.30)},   %{(3.72,0.13)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={},%{Memory size \(\displaystyle M\)},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=90},
xticklabels={10,20,40,100,200},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ylabel={ACC (\%)},
ymin=0.207334596818869, ymax=0.826252910877684,
ytick style={color=black},
ytick={0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8},
yticklabels={20,30,40,50,60,70,80}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.239599034372759)
--(axis cs:1,0.270952805627241)
--(axis cs:2,0.361675353904186)
--(axis cs:3,0.490514412785041)
--(axis cs:4,0.65900150682517)
--(axis cs:5,0.73319342111661)
--(axis cs:5,0.58319113888339)
--(axis cs:5,0.58319113888339)
--(axis cs:4,0.53162081317483)
--(axis cs:3,0.416339587214959)
--(axis cs:2,0.320832646095814)
--(axis cs:1,0.239599034372759)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.240663741878652)
--(axis cs:1,0.261369858121347)
--(axis cs:2,0.372254728113571)
--(axis cs:3,0.50465675646231)
--(axis cs:4,0.691481387295536)
--(axis cs:5,0.790365097244895)
--(axis cs:5,0.764244422755105)
--(axis cs:5,0.764244422755105)
--(axis cs:4,0.670328772704464)
--(axis cs:3,0.46668260353769)
--(axis cs:2,0.331055991886429)
--(axis cs:1,0.240663741878652)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.235467247457906)
--(axis cs:1,0.265579712542094)
--(axis cs:2,0.360101980104783)
--(axis cs:3,0.497597244200565)
--(axis cs:4,0.513972718801836)
--(axis cs:5,0.547238328540204)
--(axis cs:5,0.529725671459795)
--(axis cs:5,0.529725671459795)
--(axis cs:4,0.482284241198164)
--(axis cs:3,0.406836115799435)
--(axis cs:2,0.317198179895217)
--(axis cs:1,0.235467247457906)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.260097861289978)
--(axis cs:1,0.303615570068359)
--(axis cs:2,0.40355184674263)
--(axis cs:3,0.532415688037872)
--(axis cs:4,0.690707743167877)
--(axis cs:5,0.798120260238647)
--(axis cs:5,0.764758944511414)
--(axis cs:5,0.764758944511414)
--(axis cs:4,0.646546065807343)
--(axis cs:3,0.483370840549469)
--(axis cs:2,0.388861387968063)
--(axis cs:1,0.260097861289978)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.25527592
2 0.341254
3 0.453427
4 0.59531116
5 0.65819228
};
\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.2510168
2 0.35165536
3 0.48566968
4 0.68090508
5 0.77730476
};
\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.25052348
2 0.33865008
3 0.45221668
4 0.49812848
5 0.538482
};
\addlegendentry{Heur-GD}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.281856715679169
2 0.396206617355347
3 0.507893264293671
4 0.66862690448761
5 0.781439602375031
};
\addlegendentry{MCTS (Ours)}



==> figures/class_il_scenario/miniImagenet_acc_over_memory.tex <==
\nextgroupplot[title=Split miniImagenet,
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
minor xtick={},
minor ytick={0.025, 0.075, 0.125, 0.175},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={Memory size \(\displaystyle M\)},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xticklabel style={rotate=90},
xtick={1,2,3,4,5},
xticklabels={100,200,400,800,1600},
y grid style={white!69.0196078431373!black},
ymajorgrids, yminorgrids,
ylabel={},%{ACC},
ymin=0.0250194875900794, ymax=0.163680961167506,
ytick style={color=black},
ytick={0.0,0.05,0.1,0.15,0.2},
yticklabels={0,5,10,15,20}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.0313222818435987)
--(axis cs:1,0.0358777181564013)
--(axis cs:2,0.0383538253904577)
--(axis cs:3,0.0520830291444803)
--(axis cs:4,0.094789623249212)
--(axis cs:5,0.150202973465274)
--(axis cs:5,0.124237026534726)
--(axis cs:5,0.124237026534726)
--(axis cs:4,0.073290376750788)
--(axis cs:3,0.0441569708555197)
--(axis cs:2,0.0335661746095423)
--(axis cs:1,0.0313222818435987)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.0313590386836849)
--(axis cs:1,0.0355209613163151)
--(axis cs:2,0.03886513344562)
--(axis cs:3,0.045034926708348)
--(axis cs:4,0.0766174212255784)
--(axis cs:5,0.135689281611291)
--(axis cs:5,0.107710718388709)
--(axis cs:5,0.107710718388709)
--(axis cs:4,0.0663825787744216)
--(axis cs:3,0.041965073291652)
--(axis cs:2,0.03605486655438)
--(axis cs:1,0.0313590386836849)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.0314855663138367)
--(axis cs:1,0.0343544336861633)
--(axis cs:2,0.0430923381698826)
--(axis cs:3,0.0774133476640739)
--(axis cs:4,0.0958946944283004)
--(axis cs:5,0.0974744892773979)
--(axis cs:5,0.0704055107226021)
--(axis cs:5,0.0704055107226021)
--(axis cs:4,0.0729053055716996)
--(axis cs:3,0.0619066523359261)
--(axis cs:2,0.0359476618301174)
--(axis cs:1,0.0314855663138367)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.0332380868494511)
--(axis cs:1,0.0370019115507603)
--(axis cs:2,0.0444378703832626)
--(axis cs:3,0.0833664909005165)
--(axis cs:4,0.128646552562714)
--(axis cs:5,0.157378166913986)
--(axis cs:5,0.150621831417084)
--(axis cs:5,0.150621831417084)
--(axis cs:4,0.102633446455002)
--(axis cs:3,0.0694335028529167)
--(axis cs:2,0.0406821295619011)
--(axis cs:1,0.0332380868494511)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.0336
2 0.03596
3 0.04812
4 0.08404
5 0.13722
};
%\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.03344
2 0.03746
3 0.0435
4 0.0715
5 0.1217
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.03292
2 0.03952
3 0.06966
4 0.0844
5 0.08394
};
%\addlegendentry{Heuristic GD}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.0351199992001057
2 0.0425599999725819
3 0.0763999968767166
4 0.115639999508858
5 0.153999999165535
};
%\addlegendentry{RS-MCTS}



==> figures/class_il_scenario/notMNIST_acc_over_memory.tex <==
\nextgroupplot[title=Split notMNIST,
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={},%{Memory size \(\displaystyle M\)},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=90},
xticklabels={10,20,40,100,200},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ylabel={},%{ACC (\%)},
ymin=0.225458743774345, ymax=0.835672401123413,
ytick style={color=black},
ytick={0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8},
yticklabels={20,30,40,50,60,70,80}
]
\path [fill=color0, fill opacity=0.2, line width=1pt]
(axis cs:1,0.253195728199302)
--(axis cs:1,0.356370351800698)
--(axis cs:2,0.440226502061888)
--(axis cs:3,0.586615478105434)
--(axis cs:4,0.68543926490655)
--(axis cs:5,0.727179797674989)
--(axis cs:5,0.614241002325012)
--(axis cs:5,0.614241002325012)
--(axis cs:4,0.61583833509345)
--(axis cs:3,0.527461881894566)
--(axis cs:2,0.415446297938112)
--(axis cs:1,0.253195728199302)
--cycle;

\path [fill=color1, fill opacity=0.2, line width=1pt]
(axis cs:1,0.25642352035413)
--(axis cs:1,0.37705271964587)
--(axis cs:2,0.511336372802685)
--(axis cs:3,0.619436120812713)
--(axis cs:4,0.741949565448152)
--(axis cs:5,0.773916340300466)
--(axis cs:5,0.769029259699534)
--(axis cs:5,0.769029259699534)
--(axis cs:4,0.709001874551848)
--(axis cs:3,0.541882599187286)
--(axis cs:2,0.392921947197315)
--(axis cs:1,0.25642352035413)
--cycle;

\path [fill=color2, fill opacity=0.2, line width=1pt]
(axis cs:1,0.263747909513255)
--(axis cs:1,0.333500890486745)
--(axis cs:2,0.488109228342112)
--(axis cs:3,0.60002014707097)
--(axis cs:4,0.602947658076147)
--(axis cs:5,0.603284795039121)
--(axis cs:5,0.537684164960879)
--(axis cs:5,0.537684164960879)
--(axis cs:4,0.562598421923853)
--(axis cs:3,0.47801193292903)
--(axis cs:2,0.414494531657888)
--(axis cs:1,0.263747909513255)
--cycle;

\path [fill=color3, fill opacity=0.2, line width=1pt]
(axis cs:1,0.337080836296082)
--(axis cs:1,0.407582759857178)
--(axis cs:2,0.486506044864655)
--(axis cs:3,0.657773017883301)
--(axis cs:4,0.747565984725952)
--(axis cs:5,0.807935416698456)
--(axis cs:5,0.710279047489166)
--(axis cs:5,0.710279047489166)
--(axis cs:4,0.676063060760498)
--(axis cs:3,0.593173265457153)
--(axis cs:2,0.470134317874908)
--(axis cs:1,0.337080836296082)
--cycle;

\addplot [line width=1.0pt, color0, mark=*, mark size=1, mark options={solid}]
table {%
1 0.30478304
2 0.4278364
3 0.55703868
4 0.6506388
5 0.6707104
};
%\addlegendentry{Random}
\addplot [line width=1.0pt, color1, mark=*, mark size=1, mark options={solid}]
table {%
1 0.31673812
2 0.45212916
3 0.58065936
4 0.72547572
5 0.7714728
};
%\addlegendentry{ETS}
\addplot [line width=1.0pt, color2, mark=*, mark size=1, mark options={solid}]
table {%
1 0.2986244
2 0.45130188
3 0.53901604
4 0.58277304
5 0.57048448
};
%\addlegendentry{Heuristic GD}
\addplot [line width=1.0pt, color3, mark=*, mark size=1, mark options={solid}]
table {%
1 0.37233179807663
2 0.478320181369781
3 0.625473141670227
4 0.711814522743225
5 0.759107232093811
};
%\addlegendentry{RS-MCTS}


==> figures/policy_cifar10/bubble_rs_dataset_seed_18_ets.tex <==


\nextgroupplot[title={Replay Schedule},
height=\figheight,
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
grid=major,
xlabel={Current Task},
xmin=1.5, xmax=5.5,
xtick style={color=black},
xtick={2,3,4,5},
xticklabels={2,3,4,5},
%xticklabel style = {font=\tiny},
y grid style={white!69.0196078431373!black},
ylabel={Replayed Task},
%ylabel style={at={(-0.17,0.0)},
ymin=0.45, ymax=4.5,
ytick style={color=black},
ytick={1,2,3,4},
yticklabels={1,2,3,4},
%yticklabel style = {font=\tiny},
]
\addplot+[
mark=*,
only marks,
scatter,
scatter src=explicit,
scatter/@pre marker code/.code={%
  \expanded{%
    \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
    \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
  }%
  \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
},
visualization depends on={\thisrow{sizedata}/5 \as \perpointmarksize},
visualization depends on={value \thisrow{draw} \as \drawcolor},
visualization depends on={value \thisrow{fill} \as \fillcolor},
%visualization depends on=
%{5*cos(deg(x)) \as \perpointmarksize},
scatter/@pre marker code/.append style=
{/tikz/mark size=\perpointmarksize}
]
table[x=x, y=y, meta=sizedata]{
x  y  draw  fill  sizedata
2 1 31,119,180 31,119,180 17.841241161527712
3 1 31,119,180 31,119,180 12.6156626101008
4 1 31,119,180 31,119,180 10.300645387285055
5 1 31,119,180 31,119,180 8.920620580763856

3 2 255,127,14 255,127,14 12.6156626101008
4 2 255,127,14 255,127,14 10.300645387285055
5 2 255,127,14 255,127,14 8.920620580763856

4 3 44,160,44 44,160,44 10.300645387285055
5 3 44,160,44 44,160,44 8.920620580763856

5 4 214,39,40 214,39,40 8.920620580763856
};



==> figures/policy_cifar10/bubble_rs_dataset_seed_18_heuristic3.tex <==


\nextgroupplot[title={},
height=\figheight,
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
grid=major,
xlabel={Current Task},
xmin=1.5, xmax=5.5,
xtick style={color=black},
xtick={2,3,4,5},
xticklabels={2,3,4,5},
%xticklabel style = {font=\tiny},
y grid style={white!69.0196078431373!black},
ylabel={Replayed Task},
%ylabel style={at={(-0.17,0.0)},
ymin=0.45, ymax=4.5,
ytick style={color=black},
ytick={1,2,3,4},
yticklabels={1,2,3,4},
%yticklabel style = {font=\tiny},
]
\addplot+[
mark=*,
only marks,
scatter,
scatter src=explicit,
scatter/@pre marker code/.code={%
  \expanded{%
    \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
    \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
  }%
  \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
},
visualization depends on={\thisrow{sizedata}/5 \as \perpointmarksize},
visualization depends on={value \thisrow{draw} \as \drawcolor},
visualization depends on={value \thisrow{fill} \as \fillcolor},
%visualization depends on=
%{5*cos(deg(x)) \as \perpointmarksize},
scatter/@pre marker code/.append style=
{/tikz/mark size=\perpointmarksize}
]
table[x=x, y=y, meta=sizedata]{
x  y  draw  fill  sizedata
2 1 31,119,180 31,119,180 0.0
3 1 31,119,180 31,119,180 0.0
4 1 31,119,180 31,119,180 12.6156626101008
5 1 31,119,180 31,119,180 10.300645387285055

3 2 255,127,14 255,127,14 0.0
4 2 255,127,14 255,127,14 12.6156626101008
5 2 255,127,14 255,127,14 10.300645387285055

4 3 44,160,44 44,160,44 0.0
5 3 44,160,44 44,160,44 10.300645387285055

};


==> figures/policy_cifar10/bubble_rs_dataset_seed_19_a2c_seed_2.tex <==


\nextgroupplot[title={Replay Schedule},
height=\figheight,
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
grid=major,
xlabel={Current Task},
xmin=1.5, xmax=5.5,
xtick style={color=black},
xtick={2,3,4,5},
xticklabels={2,3,4,5},
%xticklabel style = {font=\tiny},
y grid style={white!69.0196078431373!black},
ylabel={Replayed Task},
%ylabel style={at={(-0.17,0.0)},
ymin=0.45, ymax=4.5,
ytick style={color=black},
ytick={1,2,3,4},
yticklabels={1,2,3,4},
%yticklabel style = {font=\tiny},
]
\addplot+[
mark=*,
only marks,
scatter,
scatter src=explicit,
scatter/@pre marker code/.code={%
  \expanded{%
    \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
    \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
  }%
  \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
},
visualization depends on={\thisrow{sizedata}/5 \as \perpointmarksize},
visualization depends on={value \thisrow{draw} \as \drawcolor},
visualization depends on={value \thisrow{fill} \as \fillcolor},
%visualization depends on=
%{5*cos(deg(x)) \as \perpointmarksize},
scatter/@pre marker code/.append style=
{/tikz/mark size=\perpointmarksize}
]
table[x=x, y=y, meta=sizedata]{
x  y  draw  fill  sizedata
2 1 31,119,180 31,119,180 17.841241161527712
3 1 31,119,180 31,119,180 17.841241161527712
4 1 31,119,180 31,119,180 10.300645387285055
5 1 31,119,180 31,119,180 8.920620580763856

3 2 255,127,14 255,127,14 0.0
4 2 255,127,14 255,127,14 14.567312407894388
5 2 255,127,14 255,127,14 15.450968080927584

4 3 44,160,44 44,160,44 0.0
5 3 44,160,44 44,160,44 0.0

};

==> figures/policy_cifar10/bubble_rs_dataset_seed_19_dqn_seed_2.tex <==



\nextgroupplot[title={},
height=\figheight,
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
grid=major,
xlabel={Current Task},
xmin=1.5, xmax=5.5,
xtick style={color=black},
xtick={2,3,4,5},
xticklabels={2,3,4,5},
%xticklabel style = {font=\tiny},
y grid style={white!69.0196078431373!black},
ylabel={Replayed Task},
%ylabel style={at={(-0.17,0.0)},
ymin=0.45, ymax=4.5,
ytick style={color=black},
ytick={1,2,3,4},
yticklabels={1,2,3,4},
%yticklabel style = {font=\tiny},
]
\addplot+[
mark=*,
only marks,
scatter,
scatter src=explicit,
scatter/@pre marker code/.code={%
  \expanded{%
    \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
    \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
  }%
  \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
},
visualization depends on={\thisrow{sizedata}/5 \as \perpointmarksize},
visualization depends on={value \thisrow{draw} \as \drawcolor},
visualization depends on={value \thisrow{fill} \as \fillcolor},
%visualization depends on=
%{5*cos(deg(x)) \as \perpointmarksize},
scatter/@pre marker code/.append style=
{/tikz/mark size=\perpointmarksize}
]
table[x=x, y=y, meta=sizedata]{
x  y  draw  fill  sizedata
2 1 31,119,180 31,119,180 17.841241161527712
3 1 31,119,180 31,119,180 17.841241161527712
4 1 31,119,180 31,119,180 17.841241161527712
5 1 31,119,180 31,119,180 12.6156626101008

3 2 255,127,14 255,127,14 0.0
4 2 255,127,14 255,127,14 0.0
5 2 255,127,14 255,127,14 0.0

4 3 44,160,44 44,160,44 0.0
5 3 44,160,44 44,160,44 8.920620580763856

};




==> figures/policy_cifar10/groupplot_dqn.tex <==

%\pgfplotsset{every axis title/.append style={at={(0.5,0.82)}}} %{at={(0.5,0.84)}}}
%\pgfplotsset{every tick label/.append style={font=\tiny}}
%\pgfplotsset{every major tick/.append style={major tick length=2pt}}
%\pgfplotsset{every minor tick/.append style={minor tick length=1pt}}
%\pgfplotsset{every axis x label/.append style={at={(0.5,-0.27)}}}
%\pgfplotsset{every axis y label/.append style={at={(-0.17,0.5)}}}
%\pgfplotsset{scaled x ticks=false} % switching off scientific notation for x ticks

\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}


\begin{groupplot}[group style={group size= 2 by 1, horizontal sep=1.2cm, vertical sep=1.2cm}]

\input{figures/policy_cifar10/task_acc_dataset_seed_19_dqn_seed_2}

\input{figures/policy_cifar10/bubble_rs_dataset_seed_19_dqn_seed_2}

\end{groupplot}

\end{tikzpicture}


==> figures/policy_cifar10/groupplot_heuristic3.tex <==

%\pgfplotsset{every axis title/.append style={at={(0.5,0.82)}}} %{at={(0.5,0.84)}}}
%\pgfplotsset{every tick label/.append style={font=\tiny}}
%\pgfplotsset{every major tick/.append style={major tick length=2pt}}
%\pgfplotsset{every minor tick/.append style={minor tick length=1pt}}
%\pgfplotsset{every axis x label/.append style={at={(0.5,-0.27)}}}
%\pgfplotsset{every axis y label/.append style={at={(-0.17,0.5)}}}
%\pgfplotsset{scaled x ticks=false} % switching off scientific notation for x ticks

\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}


\begin{groupplot}[group style={group size= 2 by 1, horizontal sep=1.2cm, vertical sep=1.2cm}]

\input{figures/policy_cifar10/task_acc_dataset_seed_18_heuristic3}

\input{figures/policy_cifar10/bubble_rs_dataset_seed_18_heuristic3}

\end{groupplot}

\end{tikzpicture}


==> figures/policy_cifar10/task_acc_dataset_seed_18_ets.tex <==
\nextgroupplot[title={ACC: 88.32\%},
height=\figheight,
legend cell align={left},
legend columns=1,
legend style={
  nodes={scale=0.8},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(2.65,-0.12)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={Task},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={1,2,3,4,5},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy  (\%)},
ymajorgrids,
ymin=0.7, ymax=1.01,
ytick style={color=black},
ytick={0.5,0.6,0.7,0.8,0.9,1,1.1},
yticklabels={50,60,70,80,90,100,110}
]
\addplot [line width=1.5pt, color0, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.9555
2 0.864
3 0.8995
4 0.8635
5 0.852
};
\addlegendentry{T1}
\addplot [line width=1.5pt, color1, mark=*, mark size=1.5, mark options={solid}]
table {%
2 0.97
3 0.8725
4 0.7205
5 0.8205
};
\addlegendentry{T2}
\addplot [line width=1.5pt, color2, mark=*, mark size=1.5, mark options={solid}]
table {%
3 0.981
4 0.8755
5 0.9325
};
\addlegendentry{T3}
\addplot [line width=1.5pt, color3, mark=*, mark size=1.5, mark options={solid}]
table {%
4 0.946
5 0.84
};
\addlegendentry{T4}
\addplot [line width=1.5pt, color4, mark=*, mark size=1.5, mark options={solid}]
table {%
5 0.971
};
\addlegendentry{T5}



==> figures/policy_cifar10/task_acc_dataset_seed_18_heuristic3.tex <==
\nextgroupplot[
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
title={},
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={Task Number},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0.5, ymax=1.01,
ytick style={color=black},
ytick={0.5,0.6,0.7,0.8,0.9,1,1.1}
]
\addplot [semithick, color0, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.974
2 0.899
3 0.8835
4 0.821
5 0.8405
};
%\addlegendentry{Task 1}
\addplot [semithick, color1, mark=*, mark size=1.5, mark options={solid}]
table {%
2 0.9645
3 0.809
4 0.761
5 0.8215
};
%\addlegendentry{Task 2}
\addplot [semithick, color2, mark=*, mark size=1.5, mark options={solid}]
table {%
3 0.983
4 0.888
5 0.9025
};
%\addlegendentry{Task 3}
\addplot [semithick, color3, mark=*, mark size=1.5, mark options={solid}]
table {%
4 0.955
5 0.8985
};
%\addlegendentry{Task 4}
\addplot [semithick, color4, mark=*, mark size=1.5, mark options={solid}]
table {%
5 0.9665
};
%\addlegendentry{Task 5}



==> figures/policy_cifar10/task_acc_dataset_seed_19_a2c_seed_2.tex <==
% This file was created with tikzplotlib v0.9.17.
%\begin{tikzpicture}

%\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
%\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
%\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
%\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
%\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\nextgroupplot[title={ACC: 89.75\%},
height=\figheight,
legend cell align={left},
legend columns=-1,
legend style={
  nodes={scale=0.8},
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(-0.05,1.07)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={Task},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabels={1,2,3,4,5},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy (\%)},
ymajorgrids,
ymin=0.7, ymax=1.01,
ytick style={color=black},
ytick={0.5,0.6,0.7,0.8,0.9,1,1.1},
yticklabels={50,60,70,80,90,100,110}
]
\addplot [line width=1.5pt, color0, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.973999977111816
2 0.922500014305115
3 0.909500002861023
4 0.846000015735626
5 0.882499992847443
};
%\addlegendentry{T1}
\addplot [line width=1.5pt, color1, mark=*, mark size=1.5, mark options={solid}]
table {%
2 0.966000020503998
3 0.828000009059906
4 0.755500018596649
5 0.904500007629395
};
%\addlegendentry{T2}
\addplot [line width=1.5pt, color2, mark=*, mark size=1.5, mark options={solid}]
table {%
3 0.986999988555908
4 0.920000016689301
5 0.886500000953674
};
%\addlegendentry{T3}
\addplot [line width=1.5pt, color3, mark=*, mark size=1.5, mark options={solid}]
table {%
4 0.94650000333786
5 0.840499997138977
};
%\addlegendentry{T4}
\addplot [line width=1.5pt, color4, mark=*, mark size=1.5, mark options={solid}]
table {%
5 0.97350001335144
};
%\addlegendentry{T5}
%\end{axis}

%\end{tikzpicture}


==> figures/policy_cifar10/task_acc_dataset_seed_19_dqn_seed_2.tex <==
\nextgroupplot[
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
title={},
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={Task Number},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0.5, ymax=1.01,
ytick style={color=black},
ytick={0.5,0.6,0.7,0.8,0.9,1,1.1}
]
\addplot [semithick, color0, mark=*, mark size=1.5, mark options={solid}]
table {%
1 0.973999977111816
2 0.922500014305115
3 0.909500002861023
4 0.869000017642975
5 0.867500007152557
};
%\addlegendentry{Task 1}
\addplot [semithick, color1, mark=*, mark size=1.5, mark options={solid}]
table {%
2 0.966000020503998
3 0.828000009059906
4 0.722000002861023
5 0.791999995708466
};
%\addlegendentry{Task 2}
\addplot [semithick, color2, mark=*, mark size=1.5, mark options={solid}]
table {%
3 0.986999988555908
4 0.925000011920929
5 0.855499982833862
};
%\addlegendentry{Task 3}
\addplot [semithick, color3, mark=*, mark size=1.5, mark options={solid}]
table {%
4 0.949500024318695
5 0.853999972343445
};
%\addlegendentry{Task 4}
\addplot [semithick, color4, mark=*, mark size=1.5, mark options={solid}]
table {%
5 0.970000028610229
};
%\addlegendentry{Task 5}



==> figures/single_task_replay_experiment/single_task_replay_T2.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\begin{axis}[
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={Task},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0.7, ymax=1.01,
ytick style={color=black},
ytick={0.6,0.7,0.8,0.9,1,1.1},
yticklabels={0.6,0.7,0.8,0.9,1.0,1.1}
]
\addplot [line width=1.5pt, color0, mark=*, mark size=3, mark options={solid}]
table {%
1 0.999527156352997
2 0.997730553150177
3 0.882458686828613
4 0.794799029827118
5 0.841323971748352
};
\addlegendentry{Task 1}
\addplot [line width=1.5pt, color1, mark=*, mark size=3, mark options={solid}]
table {%
2 0.995984375476837
3 0.963858962059021
4 0.868658185005188
5 0.76601368188858
};
\addlegendentry{Task 2}
\addplot [line width=1.5pt, color2, mark=*, mark size=3, mark options={solid}]
table {%
3 0.998612582683563
4 0.950907111167908
5 0.886979699134827
};
\addlegendentry{Task 3}
\addplot [line width=1.5pt, color3, mark=*, mark size=3, mark options={solid}]
table {%
4 0.999194324016571
5 0.993353486061096
};
\addlegendentry{Task 4}
\addplot [line width=1.5pt, color4, mark=*, mark size=3, mark options={solid}]
table {%
5 0.995259761810303
};
\addlegendentry{Task 5}
\addplot [line width=1.5pt, black, opacity=0.5, dashed, forget plot]
table {%
2 0
2 1.05
};
\end{axis}

\end{tikzpicture}


==> figures/single_task_replay_experiment/single_task_replay_T3.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\begin{axis}[
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={Task},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0.7, ymax=1.01,
ytick style={color=black},
ytick={0.6,0.7,0.8,0.9,1,1.1},
yticklabels={0.6,0.7,0.8,0.9,1.0,1.1}
]
\addplot [line width=1.5pt, color0, mark=*, mark size=3, mark options={solid}]
table {%
1 0.999527156352997
2 0.990638375282288
3 0.998770713806152
4 0.954420864582062
5 0.953191578388214
};
\addlegendentry{Task 1}
\addplot [line width=1.5pt, color1, mark=*, mark size=3, mark options={solid}]
table {%
2 0.995102763175964
3 0.970029354095459
4 0.915377020835876
5 0.799706101417542
};
\addlegendentry{Task 2}
\addplot [line width=1.5pt, color2, mark=*, mark size=3, mark options={solid}]
table {%
3 0.998505890369415
4 0.964674472808838
5 0.954108893871307
};
\addlegendentry{Task 3}
\addplot [line width=1.5pt, color3, mark=*, mark size=3, mark options={solid}]
table {%
4 0.999395728111267
5 0.990936577320099
};
\addlegendentry{Task 4}
\addplot [line width=1.5pt, color4, mark=*, mark size=3, mark options={solid}]
table {%
5 0.994755387306213
};
\addlegendentry{Task 5}
\addplot [line width=1.5pt, black, opacity=0.5, dashed, forget plot]
table {%
3 0
3 1.05
};
\end{axis}

\end{tikzpicture}


==> figures/single_task_replay_experiment/single_task_replay_T4.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\begin{axis}[
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={Task},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0.7, ymax=1.01,
ytick style={color=black},
ytick={0.6,0.7,0.8,0.9,1,1.1},
yticklabels={0.6,0.7,0.8,0.9,1.0,1.1}
]
\addplot [line width=1.5pt, color0, mark=*, mark size=3, mark options={solid}]
table {%
1 0.999527156352997
2 0.990638375282288
3 0.784302592277527
4 0.994799017906189
5 0.979763627052307
};
\addlegendentry{Task 1}
\addplot [line width=1.5pt, color1, mark=*, mark size=3, mark options={solid}]
table {%
2 0.995102763175964
3 0.967384934425354
4 0.902546525001526
5 0.736434817314148
};
\addlegendentry{Task 2}
\addplot [line width=1.5pt, color2, mark=*, mark size=3, mark options={solid}]
table {%
3 0.998185753822327
4 0.962860226631165
5 0.960298895835876
};
\addlegendentry{Task 3}
\addplot [line width=1.5pt, color3, mark=*, mark size=3, mark options={solid}]
table {%
4 0.998892307281494
5 0.988116860389709
};
\addlegendentry{Task 4}
\addplot [line width=1.5pt, color4, mark=*, mark size=3, mark options={solid}]
table {%
5 0.994049429893494
};
\addlegendentry{Task 5}
\addplot [line width=1.5pt, black, opacity=0.5, dashed, forget plot]
table {%
4 0
4 1.05
};
\end{axis}

\end{tikzpicture}


==> figures/single_task_replay_experiment/single_task_replay_T5.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\begin{axis}[
height=\figheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\figwidth,
x grid style={white!69.0196078431373!black},
xlabel={Task},
xmajorgrids,
xmin=0.8, xmax=5.2,
xtick style={color=black},
xtick={1,2,3,4,5},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymajorgrids,
ymin=0.7, ymax=1.01,
ytick style={color=black},
ytick={0.6,0.7,0.8,0.9,1,1.1},
yticklabels={0.6,0.7,0.8,0.9,1.0,1.1}
]
\addplot [line width=1.5pt, color0, mark=*, mark size=3, mark options={solid}]
table {%
1 0.999527156352997
2 0.990638375282288
3 0.784302592277527
4 0.645106375217438
5 0.995650112628937
};
\addlegendentry{Task 1}
\addplot [line width=1.5pt, color1, mark=*, mark size=3, mark options={solid}]
table {%
2 0.995102763175964
3 0.967384934425354
4 0.905876517295837
5 0.780019640922546
};
\addlegendentry{Task 2}
\addplot [line width=1.5pt, color2, mark=*, mark size=3, mark options={solid}]
table {%
3 0.998185753822327
4 0.969583809375763
5 0.966808974742889
};
\addlegendentry{Task 3}
\addplot [line width=1.5pt, color3, mark=*, mark size=3, mark options={solid}]
table {%
4 0.999295055866241
5 0.987814724445343
};
\addlegendentry{Task 4}
\addplot [line width=1.5pt, color4, mark=*, mark size=3, mark options={solid}]
table {%
5 0.994452834129333
};
\addlegendentry{Task 5}
\addplot [line width=1.5pt, black, opacity=0.5, dashed, forget plot]
table {%
5 0
5 1.05
};
\end{axis}

\end{tikzpicture}


==> tables/rankings_comparison_rl_experiment.tex <==
\begin{tabular}{lcccccc}
\toprule
                & \multicolumn{4}{c}{\textbf{New Task Order}}        & \multicolumn{2}{c}{\textbf{New Dataset}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-7}
\textbf{Method} & S-MNIST & S-FashionMNIST & S-notMNIST & S-CIFAR-10 & S-FashionMNIST        & S-notMNIST       \\ 
\midrule
Random          & \cellcolor{blue!15}3.98    & \textcolor{forestgreen}{3.44}           & 3.68       & 4.91       & 3.99                  & 3.94             \\
ETS             & \cellcolor{orange!20}3.82    & 4.56           & 4.44       & 5.38       & \textcolor{orange}{3.68}                  & 4.06             \\
Heur-GD         & \cellcolor{forestgreen!30}4.53    & 4.23           & 3.44       & 4.03       & \textcolor{forestgreen}{2.86}                  & 4.61             \\
Heur-LD         & 4.67    & \textcolor{orange}{3.63}           & 3.96       & 3.63       & 5.08                  & 4.96             \\
Heur-AT         & 4.38    & 3.96           & 5.5        & \textcolor{orange}{3.43}       & 3.75                  & 4.29             \\
\midrule
DQN (Ours)            & \textcolor{orange}{3.46}    & 3.65           & \textcolor{orange}{3.51}       & 3.83       & 4.42                  & \textcolor{orange}{3.4}              \\
A2C (Ours)            & \textcolor{forestgreen}{3.16}    & 4.53           & \textcolor{forestgreen}{3.47}       & \textcolor{forestgreen}{2.79}       & 4.22                  & \textcolor{forestgreen}{2.74}  \\
\bottomrule
\end{tabular}

==> tables/rankings_table_test.tex <==
\begin{tabular}{lcccccccccccccccccc}
        & \multicolumn{12}{c}{New Task Order}                                                                                                                                 & \multicolumn{6}{c}{New Dataset}                                                 \\
        & \multicolumn{3}{c}{S-MNIST}             & \multicolumn{3}{c}{S-FashionMNIST}     & \multicolumn{3}{c}{S-notMNIST}         & \multicolumn{3}{c}{S-CIFAR-10}          & \multicolumn{3}{c}{S-notMNIST}         & \multicolumn{3}{c}{S-FashionMNIST}     \\
Method  & Rank & ACC (\%)       & BWT (\%)        & Rank & ACC (\%)       & BWT (\%)       & Rank & ACC (\%)       & BWT (\%)       & Rank & ACC (\%)       & BWT (\%)        & Rank & ACC (\%)       & BWT (\%)       & Rank & ACC (\%)       & BWT (\%)       \\
Random  & 3.98 & 91.8 $\pm$ 4.7 & -9.7 $\pm$ 5.9  & 3.44 & 93.9 $\pm$ 3.8 & -5.6 $\pm$ 4.5 & 3.68 & 91.7 $\pm$ 2.8 & -4.8 $\pm$ 4.0 & 4.91 & 81.6 $\pm$ 6.1 & -17.2 $\pm$ 6.8 & 3.94 & 91.4 $\pm$ 2.7 & -5.5 $\pm$ 3.3 & 3.99 & 92.6 $\pm$ 4.7 & -6.9 $\pm$ 5.6 \\
ETS     & 3.82 & 91.8 $\pm$ 5.0 & -9.7 $\pm$ 6.3  & 4.56 & 93.5 $\pm$ 3.0 & -6.1 $\pm$ 3.3 & 4.44 & 90.4 $\pm$ 3.1 & -6.3 $\pm$ 4.4 & 5.38 & 81.0 $\pm$ 5.9 & -18.1 $\pm$ 6.3 & 4.06 & 91.5 $\pm$ 1.7 & -5.5 $\pm$ 1.9 & 3.68 & 92.8 $\pm$ 3.7 & -6.5 $\pm$ 4.8 \\
Heur-GD & 4.53 & 91.3 $\pm$ 4.3 & -10.3 $\pm$ 5.4 & 4.23 & 91.8 $\pm$ 7.9 & -8.2 $\pm$ 9.0 & 3.44 & 92.3 $\pm$ 1.5 & -4.1 $\pm$ 1.7 & 4.03 & 83.2 $\pm$ 5.0 & -15.4 $\pm$ 5.0 & 4.61 & 89.8 $\pm$ 4.8 & -7.6 $\pm$ 6.5 & 2.86 & 94.1 $\pm$ 2.8 & -5.0 $\pm$ 2.4 \\
Heur-LD & 4.67 & 91.0 $\pm$ 4.1 & -10.7 $\pm$ 5.2 & 3.63 & 93.8 $\pm$ 5.0 & -5.7 $\pm$ 5.5 & 3.96 & 91.7 $\pm$ 2.0 & -4.8 $\pm$ 1.9 & 3.63 & 83.5 $\pm$ 4.2 & -15.1 $\pm$ 4.2 & 4.96 & 89.1 $\pm$ 4.7 & -8.4 $\pm$ 6.3 & 5.08 & 90.9 $\pm$ 4.1 & -8.9 $\pm$ 4.7 \\
Heur-AT & 4.38 & 91.5 $\pm$ 4.0 & -10.1 $\pm$ 5.1 & 3.96 & 92.9 $\pm$ 4.9 & -6.8 $\pm$ 5.1 & 5.5  & 89.7 $\pm$ 2.9 & -7.1 $\pm$ 3.7 & 3.43 & 83.7 $\pm$ 4.3 & -14.8 $\pm$ 4.3 & 4.29 & 90.2 $\pm$ 4.9 & -7.0 $\pm$ 6.6 & 3.75 & 91.9 $\pm$ 7.0 & -7.6 $\pm$ 8.0 \\
DQN     & 3.46 & 93.0 $\pm$ 2.7 & -8.2 $\pm$ 3.4  & 3.65 & 94.2 $\pm$ 3.8 & -5.2 $\pm$ 3.9 & 3.51 & 91.9 $\pm$ 2.5 & -4.6 $\pm$ 2.8 & 3.83 & 83.0 $\pm$ 4.3 & -15.6 $\pm$ 4.3 & 3.4  & 91.7 $\pm$ 3.2 & -5.2 $\pm$ 4.5 & 4.42 & 92.0 $\pm$ 4.9 & -7.5 $\pm$ 5.4 \\
A2C     & 3.16 & 93.1 $\pm$ 3.7 & -8.1 $\pm$ 4.6  & 4.53 & 91.9 $\pm$ 6.2 & -8.1 $\pm$ 6.8 & 3.47 & 92.1 $\pm$ 1.8 & -4.3 $\pm$ 2.4 & 2.79 & 83.9 $\pm$ 3.8 & -14.5 $\pm$ 3.5 & 2.74 & 92.6 $\pm$ 1.6 & -4.1 $\pm$ 2.3 & 4.22 & 92.5 $\pm$ 3.4 & -6.9 $\pm$ 3.9
\end{tabular}


==> tables/table_applying_scheduling_to_recent_replay_methods.tex <==

\begin{table}[t]
\footnotesize
\centering
\caption{
    Performance comparison with ACC between scheduling methods MCTS (Ours), Random, ETS, and Heuristic combined with replay-based methods HAL, MER, and DER++. %DER, and DER++. 
    Memory sizes are $M=10$ and $M=100$ for the 5-task and 10/20-task datasets respectively. We report the mean and standard deviation averaged over 5 seeds. $^{*}$ denotes results where some seed did not converge. %Results on Heuristic where some seed did not converge is denoted by $^{*}$. 
    Applying MCTS to each method can outperform the same method using the baseline schedules. %Applying MCTS to each method can enhance the performance compared to using the baseline schedules. 
}
%\vspace{-3mm}
%\setlength{\tabcolsep}{5pt}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l l c c c c c c}
    \toprule
     & & \multicolumn{3}{c}{{\bf 5-task Datasets}} & \multicolumn{3}{c}{{\bf 10- and 20-task Datasets}} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    {\bf Method} & {\bf Schedule}  & S-MNIST & S-FashionMNIST & S-notMNIST & P-MNIST & S-CIFAR-100 & S-miniImagenet \\
    \midrule
    \multirow{4}{*}{HAL} & Random & 97.24 {\scriptsize ($\pm$ 0.70)}  & 86.74 {\scriptsize ($\pm$ 6.05)} & 93.61 {\scriptsize($\pm$ 1.31)}  & 88.49 {\scriptsize ($\pm$ 0.99)}  & 36.09 {\scriptsize ($\pm$ 1.77)} & 38.51 {\scriptsize ($\pm$ 2.22)} \\
     & ETS  & 94.02 {\scriptsize ($\pm$ 4.25)} &  95.81 {\scriptsize ($\pm$ 3.53)} & 91.01 {\scriptsize ($\pm$ 1.39)} & 88.46 {\scriptsize ($\pm$ 0.86)}  & 34.90 {\scriptsize ($\pm$ 2.02)} & 38.13 {\scriptsize ($\pm$ 1.18)} \\
    & Heuristic & 97.69 {\scriptsize ($\pm$ 0.19)} & $^{*}$74.16 {\scriptsize ($\pm$ 11.19)} & 93.64 {\scriptsize ($\pm$ 0.93)} & $^{*}$66.63 {\scriptsize ($\pm$ 28.50)} & 35.07 {\scriptsize($\pm$ 1.29)} & 39.51 {\scriptsize($\pm$ 1.49)} \\
     & Ours &  97.93 {\scriptsize ($\pm$ 0.56)} &  98.27 {\scriptsize ($\pm$ 0.17)} & 94.64 {\scriptsize ($\pm$ 0.39)} & 89.14 {\scriptsize ($\pm$ 0.74)}  & 40.22 {\scriptsize ($\pm$ 1.57)} & 41.39 {\scriptsize ($\pm$ 1.15)} \\
    \midrule 
    \multirow{4}{*}{MER} & Random & 93.07 {\scriptsize ($\pm$ 0.81)} & 85.53 {\scriptsize ($\pm$ 3.30)} & 91.13 {\scriptsize ($\pm$ 0.86)} & 75.90 {\scriptsize ($\pm$ 1.34)} & 42.96 {\scriptsize ($\pm$ 1.70)} & 31.48 {\scriptsize ($\pm$ 1.65)}  \\ 
     & ETS  & 92.89 {\scriptsize ($\pm$ 3.53)} & 96.47 {\scriptsize ($\pm$ 0.85)} &  93.80 {\scriptsize ($\pm$ 0.82)} & 73.01 {\scriptsize ($\pm$ 0.96)} & 43.38 {\scriptsize ($\pm$ 1.81)} & 33.58 {\scriptsize ($\pm$ 1.53)} \\
    & Heuristic & 94.30 {\scriptsize ($\pm$ 2.79)} & 96.91 {\scriptsize ($\pm$ 0.62)} & 90.90 {\scriptsize ($\pm$ 1.30)} &  83.86 {\scriptsize ($\pm$ 3.19)} & 40.90 {\scriptsize ($\pm$ 1.70)}  & 34.22 {\scriptsize ($\pm$ 1.93)} \\
    & Ours &  98.20 {\scriptsize ($\pm$ 0.16)} & 98.48 {\scriptsize ($\pm$ 0.26)} &  93.61 {\scriptsize ($\pm$ 0.71)} & 79.72 {\scriptsize ($\pm$ 0.71)} & 44.29 {\scriptsize ($\pm$ 0.69)} & 32.74 {\scriptsize ($\pm$ 1.29)} \\  
    %\midrule 
    %\multirow{4}{*}{DER} & Random & 98.23 {\scriptsize ($\pm$ 0.53)} & 96.56 {\scriptsize ($\pm$ 1.79)}  & 92.89 {\scriptsize ($\pm$ 0.86)} & 87.51 {\scriptsize ($\pm$ 1.10)} & 56.83 {\scriptsize ($\pm$ 0.76)} & 42.19  {\scriptsize ($\pm$ 0.67)} \\ 
    % & ETS  & 98.17 {\scriptsize ($\pm$ 0.35)} & 97.69 {\scriptsize ($\pm$ 0.58)} & 94.74 {\scriptsize ($\pm$ 1.05)} & 85.71 {\scriptsize ($\pm$ 0.75)} & 52.58 {\scriptsize ($\pm$ 1.49)} & 35.50  {\scriptsize ($\pm$ 2.84)} \\
    %& Heuristic & 94.57 {\scriptsize ($\pm$ 1.71)} & $^{*}$72.49 {\scriptsize ($\pm$ 19.32)} & $^{*}$77.88 {\scriptsize ($\pm$ 12.58)} & 81.56 {\scriptsize ($\pm$ 2.28)} & 55.75 {\scriptsize ($\pm$ 1.08)} & {\bf 43.62} {\scriptsize ($\pm$ 0.88)} \\
    % & Ours & {\bf 99.02} {\scriptsize ($\pm$ 0.10)} & {\bf 98.33} {\scriptsize ($\pm$ 0.51)} & {\bf 95.02} {\scriptsize ($\pm$ 0.33)} & {\bf 90.11} {\scriptsize ($\pm$ 0.18)} & {\bf 58.99} {\scriptsize ($\pm$ 0.98)} & 43.46  {\scriptsize ($\pm$ 0.95)}  \\  
    \midrule 
    \multirow{4}{*}{DER++} & Random & 97.90 {\scriptsize ($\pm$ 0.52)} & 97.10 {\scriptsize ($\pm$ 1.03)}  & 93.29 {\scriptsize ($\pm$ 1.43)} & 87.89 {\scriptsize ($\pm$ 1.10)} & 58.49  {\scriptsize ($\pm$ 1.44)} & 48.40  {\scriptsize ($\pm$ 0.69)} \\ 
     & ETS & 97.98 {\scriptsize ($\pm$ 0.52)} & 98.12 {\scriptsize ($\pm$ 0.40)} & 94.53 {\scriptsize ($\pm$ 1.02)} & 85.25 {\scriptsize ($\pm$ 0.88)} & 52.54  {\scriptsize ($\pm$ 1.06)} & 41.36  {\scriptsize ($\pm$ 2.90)} \\
    & Heuristic & 92.35 {\scriptsize ($\pm$ 2.42)} & $^{*}$67.31 {\scriptsize ($\pm$ 21.20)} & 93.88 {\scriptsize ($\pm$ 1.33)} & 79.17 {\scriptsize ($\pm$ 2.44)} & 56.70 {\scriptsize ($\pm$ 1.27)} & 45.73 {\scriptsize ($\pm$ 0.84)} \\
     & Ours &  98.84 {\scriptsize ($\pm$ 0.21)} &  98.38 {\scriptsize ($\pm$ 0.43)} &  94.73 {\scriptsize ($\pm$ 0.20)} &  89.84 {\scriptsize ($\pm$ 0.22)} &  59.23  {\scriptsize ($\pm$ 0.83)} &  49.45  {\scriptsize ($\pm$ 0.68)} \\
    \bottomrule
\end{tabular}
}
\vspace{-4mm}
\label{tab:results_applying_scheduling_to_recent_replay_methods}
\end{table}

\begin{comment}

\begin{table*}[t]
\footnotesize
\centering
\caption{
    Performance comparison between scheduling methods RS-MCTS (Ours), Random, ETS, and Heuristic when combining them with replay-based methods HAL, MER, DER, and DER++. %such as Hindsight Anchor Learning (HAL), Meta Experience Replay (MER), Dark Experience Replay (DER), and DER++. 
    Replay memory sizes are $M=10$ and $M=100$ for the 5-task and 10/20-task datasets respectively. We report the mean and standard deviation averaged over 5 seeds. Results on Heuristic where some seed did not converge is denoted by $^{*}$. Applying RS-MCTS to each method can enhance the performance compared to using the baseline schedules. 
}
%\vspace{-3mm}
%\setlength{\tabcolsep}{5pt}
\scalebox{0.87}{
\begin{tabular}{l l c c c c c c}
    \toprule
     & & \multicolumn{3}{c}{{\bf 5-task Datasets}} & \multicolumn{3}{c}{{\bf 10- and 20-task Datasets}} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    {\bf Method} & {\bf Schedule}  & S-MNIST & S-FashionMNIST & S-notMNIST & P-MNIST & S-CIFAR-100 & S-miniImagenet \\
    \midrule
    \multirow{4}{*}{HAL} & Random & 97.24 {\scriptsize ($\pm$ 0.70)}  & 86.74 {\scriptsize ($\pm$ 6.05)} & 93.61 {\scriptsize($\pm$ 1.31)}  & 88.49 {\scriptsize ($\pm$ 0.99)}  & 36.09 {\scriptsize ($\pm$ 1.77)} & 38.51 {\scriptsize ($\pm$ 2.22)} \\
     & ETS  & 94.02 {\scriptsize ($\pm$ 4.25)} &  95.81 {\scriptsize ($\pm$ 3.53)} & 91.01 {\scriptsize ($\pm$ 1.39)} & 88.46 {\scriptsize ($\pm$ 0.86)}  & 34.90 {\scriptsize ($\pm$ 2.02)} & 38.13 {\scriptsize ($\pm$ 1.18)} \\
    & Heuristic & 97.69 {\scriptsize ($\pm$ 0.19)} & $^{*}$74.16 {\scriptsize ($\pm$ 11.19)} & 93.64 {\scriptsize ($\pm$ 0.93)} & $^{*}$66.63 {\scriptsize ($\pm$ 28.50)} & 35.07 {\scriptsize($\pm$ 1.29)} & 39.51 {\scriptsize($\pm$ 1.49)} \\
     & Ours &  97.93 {\scriptsize ($\pm$ 0.56)} &  98.27 {\scriptsize ($\pm$ 0.17)} & 94.64 {\scriptsize ($\pm$ 0.39)} & 89.14 {\scriptsize ($\pm$ 0.74)}  & 40.22 {\scriptsize ($\pm$ 1.57)} & 41.39 {\scriptsize ($\pm$ 1.15)} \\
    \midrule 
    \multirow{4}{*}{MER} & Random & 93.07 {\scriptsize ($\pm$ 0.81)} & 85.53 {\scriptsize ($\pm$ 3.30)} & 91.13 {\scriptsize ($\pm$ 0.86)} & 75.90 {\scriptsize ($\pm$ 1.34)} & 42.96 {\scriptsize ($\pm$ 1.70)} & 31.48 {\scriptsize ($\pm$ 1.65)}  \\ 
     & ETS  & 92.89 {\scriptsize ($\pm$ 3.53)} & 96.47 {\scriptsize ($\pm$ 0.85)} & 93.80 {\scriptsize ($\pm$ 0.82)} & 73.01 {\scriptsize ($\pm$ 0.96)} & 43.38 {\scriptsize ($\pm$ 1.81)} & 33.58 {\scriptsize ($\pm$ 1.53)} \\
    & Heuristic & 94.30 {\scriptsize ($\pm$ 2.79)} & 96.91 {\scriptsize ($\pm$ 0.62)} & 90.90 {\scriptsize ($\pm$ 1.30)} & 83.86 {\scriptsize ($\pm$ 3.19)} & 40.90 {\scriptsize ($\pm$ 1.70)}  & 34.22 {\scriptsize ($\pm$ 1.93)} \\
    & Ours & 98.20 {\scriptsize ($\pm$ 0.16)} & 98.48 {\scriptsize ($\pm$ 0.26)} &  93.61 {\scriptsize ($\pm$ 0.71)} & 79.72 {\scriptsize ($\pm$ 0.71)} & 44.29 {\scriptsize ($\pm$ 0.69)} & 32.74 {\scriptsize ($\pm$ 1.29)} \\  
    \midrule 
    \multirow{4}{*}{DER} & Random & 98.23 {\scriptsize ($\pm$ 0.53)} & 96.56 {\scriptsize ($\pm$ 1.79)}  & 92.89 {\scriptsize ($\pm$ 0.86)} & 87.51 {\scriptsize ($\pm$ 1.10)} & 56.83 {\scriptsize ($\pm$ 0.76)} & 42.19  {\scriptsize ($\pm$ 0.67)} \\ 
     & ETS  & 98.17 {\scriptsize ($\pm$ 0.35)} & 97.69 {\scriptsize ($\pm$ 0.58)} & 94.74 {\scriptsize ($\pm$ 1.05)} & 85.71 {\scriptsize ($\pm$ 0.75)} & 52.58 {\scriptsize ($\pm$ 1.49)} & 35.50  {\scriptsize ($\pm$ 2.84)} \\
    & Heuristic & 94.57 {\scriptsize ($\pm$ 1.71)} & $^{*}$72.49 {\scriptsize ($\pm$ 19.32)} & $^{*}$77.88 {\scriptsize ($\pm$ 12.58)} & 81.56 {\scriptsize ($\pm$ 2.28)} & 55.75 {\scriptsize ($\pm$ 1.08)} & 43.62 {\scriptsize ($\pm$ 0.88)} \\
     & Ours & 99.02 {\scriptsize ($\pm$ 0.10)} & 98.33 {\scriptsize ($\pm$ 0.51)} & 95.02 {\scriptsize ($\pm$ 0.33)} & 90.11 {\scriptsize ($\pm$ 0.18)} & 58.99 {\scriptsize ($\pm$ 0.98)} & 43.46  {\scriptsize ($\pm$ 0.95)}  \\  
    \midrule 
    \multirow{4}{*}{DER++} & Random & 97.90 {\scriptsize ($\pm$ 0.52)} & 97.10 {\scriptsize ($\pm$ 1.03)}  & 93.29 {\scriptsize ($\pm$ 1.43)} & 87.89 {\scriptsize ($\pm$ 1.10)} & 58.49  {\scriptsize ($\pm$ 1.44)} & 48.40  {\scriptsize ($\pm$ 0.69)} \\ 
     & ETS & 97.98 {\scriptsize ($\pm$ 0.52)} & 98.12 {\scriptsize ($\pm$ 0.40)} & 94.53 {\scriptsize ($\pm$ 1.02)} & 85.25 {\scriptsize ($\pm$ 0.88)} & 52.54  {\scriptsize ($\pm$ 1.06)} & 41.36  {\scriptsize ($\pm$ 2.90)} \\
    & Heuristic & 92.35 {\scriptsize ($\pm$ 2.42)} & $^{*}$67.31 {\scriptsize ($\pm$ 21.20)} & 93.88 {\scriptsize ($\pm$ 1.33)} & 79.17 {\scriptsize ($\pm$ 2.44)} & 56.70 {\scriptsize ($\pm$ 1.27)} & 45.73 {\scriptsize ($\pm$ 0.84)} \\
     & Ours & 98.84 {\scriptsize ($\pm$ 0.21)} & 98.38 {\scriptsize ($\pm$ 0.43)} & 94.73 {\scriptsize ($\pm$ 0.20)} & 89.84 {\scriptsize ($\pm$ 0.22)} & 59.23  {\scriptsize ($\pm$ 0.83)} & 49.45  {\scriptsize ($\pm$ 0.68)} \\
    \bottomrule
\end{tabular}
}
\vspace{-3mm}
\label{tab:results_applying_scheduling_to_recent_replay_methods}
\end{table*}
\end{comment}

\begin{comment}

\begin{table*}[t]
\footnotesize
\centering
\caption{
    Comparison between RS-MCTS (Ours) and applying RS-MCTS with other continual learning method such as Hindsight Anchor Learning (HAL), Meta Experience Replay (MER), Dark Experience Replay (DER), and DER++. Memory size is set to $M=10$ and $M=100$ for Split MNIST and Permuted MNIST respectively. Results have been averaged over 5 seeds. We see that applying RS-MCTS to each CL method, except HAL, significantly outperforms the results for their corresponding Random and ETS schedule.
}
%\vspace{-3mm}
\begin{tabular}{l l c c c c c c}
    \toprule
     & & \multicolumn{3}{c}{{\bf 5-task Datasets}} & \multicolumn{3}{c}{{\bf 10- and 20-task Datasets}} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    {\bf Method} & {\bf Schedule}  & S-MNIST & S-FashionMNIST & S-notMNIST & P-MNIST & S-CIFAR-100 & S-miniImagenet \\
    \midrule
    \multirow{3}{*}{HAL} & Random & 97.24 ($\pm$ 0.70)  & 86.74 ($\pm$ 6.05) & 93.61 ($\pm$ 1.31)  & 88.49 ($\pm$ 0.99)  & 36.09 ($\pm$ 1.77) & 38.51 ($\pm$ 2.22) \\
     & ETS  & 94.02 ($\pm$ 4.25) &  95.81 ($\pm$ 3.53) & 91.01 ($\pm$ 1.39) & 88.46 ($\pm$ 0.86)  & 34.90 ($\pm$ 2.02) & 38.13 ($\pm$ 1.18) \\
    & Heuristic & 97.69 ($\pm$ 0.19) & 74.16 ($\pm$ 11.19)$^{*}$ & 93.64 ($\pm$ 0.93) & 66.63 ($\pm$ 28.50)$^{*}$ & 35.07 ($\pm$ 1.29) & 39.51 ($\pm$ 1.49) \\
     & Ours &  97.93 ($\pm$ 0.56) &  98.27 ($\pm$ 0.17) & 94.64 ($\pm$ 0.39) & 89.14 ($\pm$ 0.74)  & 40.22 ($\pm$ 1.57) & 41.39 ($\pm$ 1.15) \\
    \midrule 
    \multirow{3}{*}{MER} & Random & 93.07 $\pm$ 0.81 & 85.53 $\pm$ 3.30 & 91.13 $\pm$ 0.86 & 75.90 $\pm$ 1.34 & 42.96 $\pm$ 1.70 & 31.48 $\pm$ 1.65  \\ 
     & ETS  & 92.89 $\pm$ 3.53 & 96.47 $\pm$ 0.85 & 93.80 $\pm$ 0.82 & 73.01 $\pm$ 0.96 & 43.38 $\pm$ 1.81 & 33.58 $\pm$ 1.53 \\
    & Heuristic & 94.30 $\pm$ 2.79 & 96.91 $\pm$ 0.62 & 90.90 $\pm$ 1.30 & 83.86 $\pm$ 3.19 & 40.90 $\pm$ 1.70  & 34.22 $\pm$ 1.93 \\
    & Ours & 98.20 $\pm$ 0.16 & 98.48 $\pm$ 0.26 &  93.61 $\pm$ 0.71 & 79.72 $\pm$ 0.71 & 44.29 $\pm$ 0.69 & 32.74 $\pm$ 1.29 \\  
    \midrule 
    \multirow{3}{*}{DER} & Random & 98.23 $\pm$ 0.53 & 96.56 $\pm$ 1.79  & 92.89 $\pm$ 0.86 & 87.51 $\pm$ 1.10 & 56.83 $\pm$ 0.76 & 42.19  $\pm$ 0.67 \\ 
     & ETS  & 98.17 $\pm$ 0.35 & 97.69 $\pm$ 0.58 & 94.74 $\pm$ 1.05 & 85.71 $\pm$ 0.75 & 52.58 $\pm$ 1.49 & 35.50  $\pm$ 2.84 \\
    & Heuristic & 94.57 $\pm$ 1.71 & 72.49 $\pm$ 19.32$^{*}$ & 77.88 $\pm$ 12.58$^{*}$ & 81.56 $\pm$ 2.28 & 55.75 $\pm$ 1.08 & 43.62 $\pm$ 0.88 \\
     & Ours & 99.02 $\pm$ 0.10 & 98.33 $\pm$ 0.51 & 95.02 $\pm$ 0.33 & 90.11 $\pm$ 0.18 & 58.99 $\pm$ 0.98 & 43.46  $\pm$ 0.95  \\  
    \midrule 
    \multirow{3}{*}{DER++} & Random & 97.90 $\pm$ 0.52 & 97.10 $\pm$ 1.03  & 93.29 $\pm$ 1.43 & 87.89 $\pm$ 1.10 & 58.49  $\pm$ 1.44 & 48.40  $\pm$ 0.69 \\ 
     & ETS & 97.98 $\pm$ 0.52 & 98.12 $\pm$ 0.40 & 94.53 $\pm$ 1.02 & 85.25 $\pm$ 0.88 & 52.54  $\pm$ 1.06 & 41.36  $\pm$ 2.90 \\
    & Heuristic & 92.35 $\pm$ 2.42 & 67.31 $\pm$ 21.20$^{*}$ & 93.88 $\pm$ 1.33 & 79.17 $\pm$ 2.44 & 56.70 $\pm$ 1.27 & 45.73 $\pm$ 0.84 \\
     & Ours & 98.84 $\pm$ 0.21 & 98.38 $\pm$ 0.43 & 94.73 $\pm$ 0.20 & 89.84 $\pm$ 0.22 & 59.23  $\pm$ 0.83 & 49.45  $\pm$ 0.68 \\
    \bottomrule
\end{tabular}
\vspace{-3mm}
\label{tab:results_applying_scheduling_to_recent_replay_methods}
\end{table*}
\end{comment}

==> tables/table_efficiency_replay_scheduling.tex <==


\begin{table}[t]
%\scriptsize
\centering
\caption{
Accuracy comparison in the 1 sample/class memory setting evaluated across all datasets. %We use 'S' and 'P' as short for 'Split' and 'Permuted' for the datasets. 
MCTS has memory size $M=2$ and $M=50$ for the 5-task and 10/20-task datasets respectively. The baselines replay all available memory samples. We report the mean and standard deviation averaged over 5 seeds. MCTS performs on par with the best baselines on all datasets except S-CIFAR-100. 
}
%\vspace{-3mm}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l c c c c c c}
    \toprule
     & \multicolumn{3}{c}{{\bf 5-task Datasets}} & \multicolumn{3}{c}{{\bf 10- and 20-task Datasets}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    {\bf Method} & S-MNIST & S-FashionMNIST & S-notMNIST & P-MNIST & S-CIFAR-100 & S-miniImagenet \\
    \midrule 
    Random & 92.56 {\scriptsize ($\pm$ 2.90)} & 92.70 {\scriptsize ($\pm$ 3.78)} & 89.53 {\scriptsize ($\pm$ 3.96)} & 70.02 {\scriptsize ($\pm$ 1.76)} & 48.62 {\scriptsize ($\pm$ 1.02)} & 48.85 {\scriptsize ($\pm$ 1.38)} \\
    A-GEM  & 94.97 {\scriptsize ($\pm$ 1.50)} & 94.81 {\scriptsize ($\pm$ 0.86)} & 92.27 {\scriptsize ($\pm$ 1.16)} & 64.71 {\scriptsize ($\pm$ 1.78)}  & 42.22 {\scriptsize ($\pm$ 2.13)} &  32.06 {\scriptsize ($\pm$ 1.83)}  \\
    ER-Ring & 94.94 {\scriptsize ($\pm$ 1.56)} & 95.83 {\scriptsize ($\pm$ 2.15)} & 91.10 {\scriptsize ($\pm$ 1.89)} & 69.73 {\scriptsize ($\pm$ 1.13)} &  53.93 {\scriptsize ($\pm$ 1.13)} & 49.82 {\scriptsize ($\pm$ 1.69)}  \\
    Uniform &  95.77 {\scriptsize ($\pm$ 1.12)} & 97.12 {\scriptsize ($\pm$ 1.57)} & 92.14 {\scriptsize ($\pm$ 1.45)} & 69.85 {\scriptsize ($\pm$ 1.01)} & 52.63 {\scriptsize ($\pm$ 1.62)}  & 50.56 {\scriptsize ($\pm$ 1.07)}  \\
    \midrule 
    RS-MCTS (Ours) & 96.07 {\scriptsize ($\pm$ 1.60)} &  97.17 {\scriptsize ($\pm$ 0.78)} & 93.41 {\scriptsize ($\pm$ 1.11)} & 72.52 {\scriptsize ($\pm$ 0.54)} & 51.50 {\scriptsize ($\pm$ 1.19)} & 50.70 {\scriptsize ($\pm$ 0.54)} \\
    \bottomrule
\end{tabular}
}
\vspace{-4mm}
\label{tab:efficiency_of_replay_scheduling_all_datasets}
\end{table}

\begin{comment}


\begin{table}[t]
\footnotesize %\scriptsize
\centering
%\vspace{-4mm}
\caption{
Performance comparison with ACC averaged over 5 seeds in the 1 ex/class %example per class 
memory setting evaluated across all datasets. %We use 'S' and 'P' as short for 'Split' and 'Permuted' for the datasets. 
RS-MCTS (Ours) has replay memory size $M=2$ and $M=50$ for the 5-task and 10/20-task datasets respectively. The baselines replay all available memory samples. 
%We report the mean and standard deviation averaged over 5 seeds. 
RS-MCTS performs on par with the best baselines on all datasets except S-CIFAR-100.
}
%\scalebox{0.89}{
\begin{tabular}{l c c c}
    \toprule
     & \multicolumn{3}{c}{{\bf 5-task Datasets}} \\ 
    \cmidrule(lr){2-4} 
    {\bf Method} & S-MNIST & S-FashionMNIST & S-notMNIST \\
    \midrule 
    Random & 92.56 ($\pm$ 2.90) & 92.70 ($\pm$ 3.78) & 89.53 ($\pm$ 3.96)  \\
    A-GEM  & 94.97 ($\pm$ 1.50) & 94.81 ($\pm$ 0.86) & 92.27 ($\pm$ 1.16)   \\
    ER-Ring & 94.94 ($\pm$ 1.56) & 95.83 ($\pm$ 2.15) & 91.10 ($\pm$ 1.89)   \\
    Uniform &  95.77 ($\pm$ 1.12) & 97.12 ($\pm$ 1.57) & 92.14 ($\pm$ 1.45)   \\
    \midrule 
    Ours & 96.07 ($\pm$ 1.60) &  97.17 ($\pm$ 0.78) & 93.41 ($\pm$ 1.11)  \\
    \midrule \midrule 
    & \multicolumn{3}{c}{{\bf 10- and 20-task Datasets}} \\
    \cmidrule(lr){2-4}
    {\bf Method} & P-MNIST & S-CIFAR-100 & S-miniImagenet \\
    \midrule 
    Random & 70.02 ($\pm$ 1.76) & 48.62 ($\pm$ 1.02) & 48.85 ($\pm$ 1.38) \\
    A-GEM & 64.71 ($\pm$ 1.78)  & 42.22 ($\pm$ 2.13) &  32.06 ($\pm$ 1.83) \\ 
    ER-Ring & 69.73 ($\pm$ 1.13) & 53.93 ($\pm$ 1.13) & 49.82 ($\pm$ 1.69) \\
    Uniform & 69.85 ($\pm$ 1.01) & 52.63 ($\pm$ 1.62)  & 50.56 ($\pm$ 1.07) \\
    \midrule
    Ours & 72.52 ($\pm$ 0.54) & 51.50 ($\pm$ 1.19) & 50.70 ($\pm$ 0.54) \\
    \bottomrule
\end{tabular}
%}
%\vspace{-6mm}
\label{tab:efficiency_of_replay_scheduling_all_datasets}
\end{table}
\end{comment}

%\begin{comment}

%\end{comment}



==> tables/table_memory_selection_new.tex <==
\begin{tabular}{llcccccc}
\toprule
                                   &                 & \multicolumn{2}{c}{\textbf{Split MNIST}} & \multicolumn{2}{c}{\textbf{Split FashionMNIST}} & \multicolumn{2}{c}{\textbf{Split notMNIST}} \\ \midrule
\textbf{Memory}                 & \textbf{Schedule} & ACC (\%)            & BWT (\%)           & ACC (\%)               & BWT (\%)               & ACC (\%)             & BWT (\%)             \\ \midrule
Offline                            & Joint           & 99.75 $\pm$ 0.06      & 0.01 $\pm$ 0.06      & 99.34 $\pm$ 0.08         & -0.01 $\pm$ 0.14         & 96.12 $\pm$ 0.57       & -0.21 $\pm$ 0.71       \\ 
Uniform & BFS & 98.28 $\pm$ 0.49 & -1.84 $\pm$ 0.63 & 98.51 $\pm$ 0.23 & -1.03 $\pm$ 0.28 & 95.54 $\pm$ 0.67 & -1.04 $\pm$ 0.87 \\ \midrule
%\multirow{5}{*}{Uniform}           & BFS             & 98.28 $\pm$ 0.49      & -1.84 $\pm$ 0.63     & 98.51 $\pm$ 0.23         & -1.03 $\pm$ 0.28         & 95.54 $\pm$ 0.67       & -1.04 $\pm$ 0.87       \\
\multirow{4}{*}{Uniform}                                   & Random          & 94.91 $\pm$ 2.52      & -6.13 $\pm$ 3.16     & 95.89 $\pm$ 2.03         & -4.33 $\pm$ 2.55         & 91.84 $\pm$ 1.48       & -5.37 $\pm$ 2.12       \\
                                   & ETS             & 94.02 $\pm$ 4.25      & -7.22 $\pm$ 5.33     & 95.81 $\pm$ 3.53         & -4.45 $\pm$ 4.34         & 91.01 $\pm$ 1.39       & -6.16 $\pm$ 1.82       \\
                                   & Heur-GD         & 96.02 $\pm$ 2.32      & -4.64 $\pm$ 2.90     & 97.09 $\pm$ 0.62         & -2.82 $\pm$ 0.84         & 91.26 $\pm$ 3.99       & -6.06 $\pm$ 4.70       \\
                                   & MCTS            & 97.93 $\pm$ 0.56      & -2.27 $\pm$ 0.71     & 98.27 $\pm$ 0.17         & -1.29 $\pm$ 0.20         & 94.64 $\pm$ 0.39       & -1.47 $\pm$ 0.79       \\ \midrule
\multirow{4}{*}{k-means}  & Random          & 92.65 $\pm$ 1.38      & -8.96 $\pm$ 1.74     & 93.11 $\pm$ 2.75         & -7.76 $\pm$ 3.42         & 93.11 $\pm$ 1.01       & -3.78 $\pm$ 1.43       \\
                                   & ETS             & 92.89 $\pm$ 3.53      & -8.66 $\pm$ 4.42     & 96.47 $\pm$ 0.85         & -3.55 $\pm$ 1.07         & 93.80 $\pm$ 0.82       & -2.84 $\pm$ 0.81       \\
                                   & Heur-GD         & 96.28 $\pm$ 1.68      & -4.32 $\pm$ 2.11     & 95.78 $\pm$ 1.50         & -4.46 $\pm$ 1.87         & 91.75 $\pm$ 0.94       & -5.60 $\pm$ 2.07       \\
                                   & MCTS            & 98.20 $\pm$ 0.16      & -1.94 $\pm$ 0.22     & 98.48 $\pm$ 0.26         & -1.04 $\pm$ 0.31         & 93.61 $\pm$ 0.71       & -3.11 $\pm$ 0.55       \\ \midrule
\multirow{4}{*}{k-center} & Random          & 95.48 $\pm$ 0.82      & -5.40 $\pm$ 1.05     & 93.24 $\pm$ 2.84         & -7.64 $\pm$ 3.51         & 91.70 $\pm$ 1.94       & -5.33 $\pm$ 2.80       \\
                                   & ETS             & 94.84 $\pm$ 1.40      & -6.20 $\pm$ 1.77     & 97.28 $\pm$ 0.50         & -2.58 $\pm$ 0.66         & 91.08 $\pm$ 2.48       & -6.39 $\pm$ 3.46       \\
                                   & Heur-GD         & 94.55 $\pm$ 2.79      & -6.47 $\pm$ 3.50     & 94.08 $\pm$ 3.72         & -6.59 $\pm$ 4.57         & 92.06 $\pm$ 1.20       & -4.70 $\pm$ 2.09       \\
                                   & MCTS            & 98.24 $\pm$ 0.36      & -1.93 $\pm$ 0.44     & 98.06 $\pm$ 0.35         & -1.59 $\pm$ 0.45         & 94.26 $\pm$ 0.37       & -1.97 $\pm$ 1.02       \\ \midrule
\multirow{4}{*}{MoF}             & Random          & 96.96 $\pm$ 1.34      & -3.57 $\pm$ 1.69     & 96.39 $\pm$ 1.69         & -3.66 $\pm$ 2.17         & 93.09 $\pm$ 1.40       & -3.70 $\pm$ 1.76       \\
                                   & ETS             & 97.04 $\pm$ 1.23      & -3.46 $\pm$ 1.50     & 96.48 $\pm$ 1.33         & -3.55 $\pm$ 1.73         & 92.64 $\pm$ 0.87       & -4.57 $\pm$ 1.59       \\
                                   & Heur-GD         & 96.46 $\pm$ 2.41      & -4.09 $\pm$ 3.01     & 95.84 $\pm$ 0.89         & -4.39 $\pm$ 1.15         & 93.24 $\pm$ 0.77       & -3.48 $\pm$ 1.37       \\
                                   & MCTS            & 98.37 $\pm$ 0.24      & -1.70 $\pm$ 0.28     & 97.84 $\pm$ 0.32         & -1.81 $\pm$ 0.39         & 94.62 $\pm$ 0.42       & -1.80 $\pm$ 0.56       \\ 
\bottomrule
\toprule
                          &         & \multicolumn{2}{c}{\textbf{Permuted MNIST}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{Split miniImagenet}} \\ \midrule 
\textbf{Memory}                 & \textbf{Schedule}  & ACC (\%)        & BWT (\%)         & ACC (\%)         & BWT (\%)         & ACC (\%)          & BWT (\%)           \\ \midrule 
Offline                   & Joint   & 95.34 $\pm$ 0.13  & 0.17 $\pm$ 0.18    & 84.73 $\pm$ 0.81   & -1.06 $\pm$ 0.81   & 74.03 $\pm$ 0.83    & 9.70 $\pm$ 0.68      \\ \midrule 
\multirow{4}{*}{Uniform}  & Random  & 72.59 $\pm$ 1.52  & -25.71 $\pm$ 1.76  & 53.76 $\pm$ 1.80   & -35.11 $\pm$ 1.93  & 49.89 $\pm$ 1.03    & -14.79 $\pm$ 1.14    \\
                          & ETS     & 71.09 $\pm$ 2.31  & -27.39 $\pm$ 2.59  & 47.70 $\pm$ 2.16   & -41.69 $\pm$ 2.37  & 46.97 $\pm$ 1.24    & -18.32 $\pm$ 1.34    \\
                          & Heur-GD & 76.68 $\pm$ 2.13  & -20.82 $\pm$ 2.41  & 57.31 $\pm$ 1.21   & -30.76 $\pm$ 1.45  & 49.66 $\pm$ 1.10    & -12.04 $\pm$ 0.59    \\
                          & MCTS    & 76.34 $\pm$ 0.98  & -21.21 $\pm$ 1.16  & 56.60 $\pm$ 1.13   & -31.39 $\pm$ 1.11  & 50.20 $\pm$ 0.72    & -13.46 $\pm$ 1.22    \\ \midrule 
\multirow{4}{*}{k-means}  & Random  & 71.91 $\pm$ 1.24  & -26.45 $\pm$ 1.34  & 53.20 $\pm$ 1.44   & -35.77 $\pm$ 1.31  & 49.96 $\pm$ 1.46    & -14.81 $\pm$ 1.18    \\
                          & ETS     & 69.40 $\pm$ 1.32  & -29.23 $\pm$ 1.47  & 47.51 $\pm$ 1.14   & -41.77 $\pm$ 1.30  & 45.82 $\pm$ 0.92    & -19.53 $\pm$ 1.10    \\
                          & Heur-GD & 75.57 $\pm$ 1.18  & -22.11 $\pm$ 1.22  & 54.31 $\pm$ 3.94   & -33.80 $\pm$ 4.24  & 49.25 $\pm$ 1.00    & -12.92 $\pm$ 1.22    \\
                          & MCTS    & 77.74 $\pm$ 0.80  & -19.66 $\pm$ 0.95  & 56.95 $\pm$ 0.92   & -30.92 $\pm$ 0.83  & 50.47 $\pm$ 0.85    & -13.31 $\pm$ 1.24    \\ \midrule 
\multirow{4}{*}{k-center} & Random  & 71.39 $\pm$ 1.87  & -27.04 $\pm$ 2.05  & 48.29 $\pm$ 2.11   & -40.88 $\pm$ 2.28  & 44.40 $\pm$ 1.35    & -20.03 $\pm$ 1.31    \\
                          & ETS     & 69.11 $\pm$ 1.69  & -29.58 $\pm$ 1.81  & 44.13 $\pm$ 1.06   & -45.28 $\pm$ 1.04  & 41.35 $\pm$ 1.23    & -23.71 $\pm$ 1.45    \\
                          & Heur-GD & 74.33 $\pm$ 2.00  & -23.45 $\pm$ 2.27  & 50.32 $\pm$ 1.97   & -37.99 $\pm$ 2.14  & 44.13 $\pm$ 0.95    & -18.26 $\pm$ 1.05    \\
                          & MCTS    & 76.55 $\pm$ 1.16  & -21.06 $\pm$ 1.32  & 51.37 $\pm$ 1.63   & -37.01 $\pm$ 1.62  & 46.76 $\pm$ 0.96    & -16.56 $\pm$ 0.90    \\ \midrule 
\multirow{4}{*}{MoF}      & Random  & 78.80 $\pm$ 1.07  & -18.79 $\pm$ 1.16  & 62.35 $\pm$ 1.24   & -26.33 $\pm$ 1.25  & 56.02 $\pm$ 1.11    & -7.99 $\pm$ 1.13     \\
                          & ETS     & 77.62 $\pm$ 1.12  & -20.10 $\pm$ 1.26  & 60.43 $\pm$ 1.17   & -28.22 $\pm$ 1.26  & 56.12 $\pm$ 1.12    & -8.93 $\pm$ 0.83     \\
                          & Heur-GD & 77.27 $\pm$ 1.45  & -20.15 $\pm$ 1.63  & 55.60 $\pm$ 2.70   & -32.57 $\pm$ 2.77  & 52.30 $\pm$ 0.59    & -9.61 $\pm$ 0.67     \\
                          & MCTS    & 81.58 $\pm$ 0.75  & -15.41 $\pm$ 0.86  & 64.22 $\pm$ 0.65   & -23.48 $\pm$ 1.02  & 57.70 $\pm$ 0.51    & -5.31 $\pm$ 0.55    \\
\bottomrule
\end{tabular}
